Interval Universal Approximation for Neural Networks

To verify safety and robustness of neural networks, researchers have successfully applied abstract interpretation, primarily using the interval abstract domain. In this paper, we study the theoretical power and limits of the interval domain for neural-network verification. First, we introduce the interval universal approximation (IUA) theorem. IUA shows that neural networks not only can approximate any continuous function $f$ (universal approximation) as we have known for decades, but we can find a neural network, using any well-behaved activation function, whose interval bounds are an arbitrarily close approximation of the set semantics of $f$ (the result of applying $f$ to a set of inputs). We call this notion of approximation interval approximation. Our theorem generalizes the recent result of Baader et al. (2020) from ReLUs to a rich class of activation functions that we call squashable functions. Additionally, the IUA theorem implies that we can always construct provably robust neural networks under $\ell_\infty$-norm using almost any practical activation function. Second, we study the computational complexity of constructing neural networks that are amenable to precise interval analysis. This is a crucial question, as our constructive proof of IUA is exponential in the size of the approximation domain. We boil this question down to the problem of approximating the range of a neural network with squashable activation functions. We show that the range approximation problem (RA) is a $\Delta_2$-intermediate problem, which is strictly harder than $\mathsf{NP}$-complete problems, assuming $\mathsf{coNP}\not\subset \mathsf{NP}$. As a result, IUA is an inherently hard problem: No matter what abstract domain or computational tools we consider to achieve interval approximation, there is no efficient construction of such a universal approximator.

==> bump.tex <==




\section{Proof Step 1: Function slicing}\label{sec:step1}

Let  $f: C \rightarrow \mathbb{R}$ be the continuous function we need to approximate, as per AUA theorem statement (\cref{thm:main}).
In the first step of the proof, we will \emph{slice} $f$ into a sequence of functions $f_0,\ldots,f_K$,
each of which encodes the behavior of $f$ on a small interval of its range.
In the next steps of the proof, we will approximate each $f_i$ using a neural network;
since each $f_i$ operates on a small range, a coarse approximation of one $f_i$ leads to a small approximation error.

\paragraph{Slicing the range}
In what follows, without loss of generality, we can assume that $\min f(C) = 0$.\footnote{Otherwise, we can shift $f$ such that $\min f(C) = 0$.}
Let $u = \max f(C)$. 
In other words, the range of $f$ is $[0,u]$.
Note that the range of $f$ is bounded due to its continuity and compactness of $C$. 

% As stated in the statement of the AUA theorem (\cref{thm:main}),
% for any given $f$ and $\delta$, we will construct a neural network $N$ that $\delta$-abstractly approximates $f$.

Let $\unit = \frac{\delta}{3}$. 
%Then $\delta = 3\unit$. 
We call $\unit$ a unit; in~\cref{thm:main}, we have 3 units of freedom when constructing $\nn$; that is, we can afford $3$ units  of error
in our abstract approximation.
We first partition the range of $f$, $[0, u]$, into 
multiple small intervals with size $\unit$, i.e., 
\[\left[0, \unit\right],\left[\unit, 2\unit\right], \ldots, \left[K\unit, u\right]\] 
where 
$K = \floor{u/\unit}$.
We will call each such interval a \emph{slice}.
We will say $i$th slice, for $i \in \{0,\ldots,K\}$, to denote slice
$[i\unit, (i+1)\unit]$. 

\paragraph{Constructing function slices}
We will decompose $f$ into a sequence of 
\emph{function slices} $f_i$, whose values are restricted to $\left[0, \unit\right]$. The sum of the sequence of function slices 
is $f$. 
The following example shows what a function slice $f_i$ looks like.



\begin{example}
    \cref{fig:f}
    shows a function $f(x) = sin(2x) + 1$
    that we wish to approximate with precision $\delta=1.2$.
    %
    We therefore use slices of size $\unit = 0.4$ to divide the range $[0,2]$, as shown in \cref{fig:slice_f}. 
    This results in five functions, $f_0,\ldots,f_4$.
    Functions $f_0$ and $f_3$ are shown in \cref{fig:single_slice0,fig:single_slice3}, respectively.
    Observe how the function slices $f_0$ and $f_3$  are shifted down to the $x$-axis, such that their range is $[0,\unit]$.
    \end{example}


% As mentioned above, we will construct 
% a small neural network $n_i$ to approximate $f_i$, and for each $B\subseteq C$, there are at most 4 $n_i$'s that could possibly lose precision
% (see the highlighted terms and cases 4 and 5 in the proof of theorem~\ref{thm:simple} ).Three slices increase the lower bound of the interval in 
% the result of the abstract interpretation by $\delta/3$, and one slice decreases the upper bound by $\delta/3$.
% In fact, we can choose any size smaller than or equal to $\delta/2$ for the simplified network, i.e., if we use $\delta/2$, the inequality is sharp for the 
% simplified network. However, we will need extra space for loss of precision introduced by the general activation function (because the activation function has limits,
% we can control the range of the function value but the actual value might not be singleton), so we choose $\delta/3$, which is sufficient for our need throughout the paper.
%\\



\input{ill_step1}


Formally, the sequence of functions $f_i: C \to [0,\unit]$, for $i\in\{0,\ldots,K\}$, is:
\[ 
  f_i(\bx)=\begin{cases}
               f(\bx) - i \unit, & i \unit < f(\bx) \leq (i + 1)\unit \\
               0, & f(\bx) \leq i\unit \\
               \unit, &(i+1) \unit < f(\bx)
            \end{cases}
\]



The following lemma shows that
 the sum of the function slices
is equivalent to $f$.



\begin{lemma}\label{lem:slice_f}
        $\sum_{i = 0}^K f_i(\bx) = f(\bx)$, where $\bx\in C$.
\end{lemma}



\paragraph{Why slice $f$, and why $\unit$}
%
In the next two steps of the proof,
we will approximate each function $f_i$
using a small neural network separately,
and then take their sum.
The reason we perform the slicing is to limit
precision loss due to our approximation.
To give some intuition,
consider a concrete input $\bx$.
Only one of the function slices $f_i$
will produce a non-extremal behavior on $\bx$, i.e.,
$f_i(\bx) \in \left(0,\unit\right)$; 
all other function slices will output $0$ or $\unit$.
So, even if we have a discrete approximation $\hat{f}_i$
of each $f_i$ that returns $0$ or $\unit$ for any $\bx$ (whichever is closer to $f(\bx)$),
then $|f(\bx) - \sum_i \hat{f}_i(\bx)| \leq \unit$.
%
%

In our construction, we additionally control the loss of precision
due to limit-bounded activation functions, ensuring their error is at most $\unit$.
%
Further, as we shall show, only a fixed number of slices will lose precision due to abstract interpretation,
resulting in additional precision loss of $2\unit$.
This creates a total precision loss of $3\unit = \delta$.
%\todo{remove the four slices part somehow}

%\zw{I think if we say that error due to limit-bounded activation function is $\unit$, then 
%we might want to change $\lprec$ from $\frac{1}{2|\cells|}$ to $\frac{1}{|\cells|}$ just to be consistent.}
%\aws{as u like}



% As mentioned above, we will construct 
% a small neural network $n_i$ to approximate $f_i$, and for each $B\subseteq C$, there are at most 4 $n_i$'s that could possibly lose precision
% (see the highlighted terms and cases 4 and 5 in the proof of theorem~\ref{thm:simple} ).Three slices increase the lower bound of the interval in 
% the result of the abstract interpretation by $\delta/3$, and one slice decreases the upper bound by $\delta/3$.
% In fact, we can choose any size smaller than or equal to $\delta/2$ for the simplified network, i.e., if we use $\delta/2$, the inequality is sharp for the 
% simplified network. However, we will need extra space for loss of presicion introduced by the general activation function (because the activation function has limits,
% we can control the range of the function value but the actual value might not be singleton), so we choose $\delta/3$, which is sufficient for our need throughout the paper.

% We will construct a step function $n_i$ to approximate each $f_i$ and then take the sum of these piecewise linear functions.


\section{Proof Step 2: Grids and indicator functions}\label{sec:step2}

We have sliced the function $f: C \to \R$ into a sequence of functions $f_0,\ldots,f_K$.
In this step of the proof, we will begin the process of approximating 
each such function $f_i$ using a neural network.
Specifically, we will divide the domain $C$ into a grid,
and proceed by constructing a neural network that tells us
whether we are in a specific region in the grid. 
% The grid on $C$  forms an approximation for the interval domain. 
% As a result, we build an 
% indicator function for each box in $C$, the domain of $f$, with appropriate granularity.

\begin{wrapfigure}{r}{.3\textwidth}
    \vspace{-.5em}
    \begin{subfigure}{.3\textwidth}
        \centering
        \begin{tikzpicture}
          \begin{axis}[
                axis lines=middle,
                xmax=5.2,
                xmin=0,
                ymin=0,
                ymax=0.55,
                ytick={0,.4},
                xtick={10,20},
                height=0.4cm,
                width=3cm
            ]
          
            \addplot [domain=-1:5, samples=100, thick, blue] {max(min(sin(deg(2*x))+1, 1.6), 1.2)-1.2};
      
          
          \end{axis}
          %\draw [dashed] (0,1) -- (1,1);
        \end{tikzpicture}      
      \end{subfigure}

\begin{subfigure}{.3\textwidth}
    \centering
    \begin{tikzpicture}
      \begin{axis}[
            axis lines=middle,
            xmax=5.2,
            xmin=0,
            ymin=0,
            ymax=0.55,
            ytick={0,.4},
            xtick={0,1,2,3,4,5},
            height=0.4cm,
            width=3cm
        ]
      
        %\addplot [domain=-1:9, samples=100, thick, blue] {max(min(sin(deg(2*x))+1, 1.6), 1.2)};
        \addplot [domain=0:0.4, very thick, red] {0.01};
        \addplot [domain=0.4:1.2, thick, red] {1.6 - 1.2};
        \addplot [domain=1.2:1.6, thick, red] {0.01};
        \addplot [domain=1.6:3.2, thick, red] {0.01};
        \addplot [domain=3.2:3.6, thick, red] {0.01};
        \addplot [domain=3.6:4.4, thick, red] {1.6 - 1.2};
        \addplot [domain=4.4:4.8, thick, red] {0.01};
        \addplot [domain=4.8:5.0, thick, red] {0.01};
        % \pgfplotsinvokeforeach{0.2,0.4,...,5}{\addplot[mark=none,gray] coordinates { (#1,0) (#1,2) };}
        
      \end{axis}
      %\draw [dashed] (0,1) -- (1,1);
    \end{tikzpicture}
  \end{subfigure}
  \vspace{-1em}
  \caption{$f_3$ approximation}\label{fig:approx}
\end{wrapfigure}
\paragraph{Rationale}
Recall that the range of a function slice $f_i$ is $[0,\unit]$.
The value of $f_i(\bx)$ is $\unit$ if the value of $f(\bx)$ is greater than  $(i+1)\unit$.
We will coarsely approximate $f_i$ by only considering its extremal behavior;
that is, we will construct a function that roughly looks
like this:
\emph{if $\bx$ is in a region where $f(\bx) \geq (i+1)\unit$, then  approximation should return $\unit$;
otherwise, return 0.}
%
Thus, we need to be able to \emph{check} whether $\bx$ is in a specific region of the input domain $C$.
This is the purpose of this step of the proof: to construct a neural network that performs the check.
%
These regions will be box-shaped, and therefore our neural network will need to approximate an \emph{indicator} function over box-shaped sets.

\begin{example}
    \cref{fig:approx} shows slice $f_3$ from \cref{fig:single_slice3} and an approximation of its extremal behaviors  (bottom).
    This is meant as an illustration and not 
    exactly what our construction produces.
\end{example}


\paragraph{Outline of proof step 2}
In \cref{sec:step2grid},  we begin by describing how to divide the domain $C$ into a set of box-shaped regions.
In \cref{sec:step2int}, we provide an intuitive explanation of our approximation of indicator functions using activation functions.
In \cref{sec:step21d}, we describe how to approximate indicator functions for 1-dimensional boxes.
In \cref{sec:step2md}, we describe how to approximate indicator functions for $m$-dimensional boxes.



\subsection{Constructing an $\epsilon$-grid}\label{sec:step2grid}
We will now construct an $\epsilon$-\emph{grid} over the domain $C$.
The grid divides the domain $C$ into sub-regions,
for which we will construct indicator functions that will be used to approximate each slice $f_i$ (in \cref{sec:step3}).
The more finer-grained the resolution of the grid, $\epsilon$, the better the approximation of $f_i$.
We begin by discussing our choice of $\epsilon$.
%

\input{ill_step2_grid}

\paragraph{Grid resolution}
Because $C \subset \R^m$ is compact and $f$ is continuous, then $f$ is uniformly continuous on $C$ (following Heine--Cantor, \cref{thm:hc}). Thus, by definition of uniform continuity, there exists $\epsilon > 0$
such that 
\[
    \text{if } \norm{\bx - \by}_\infty \leq \epsilon, \text{ then }  |f(\bx) - f(\by)| < \unit
\]

Pick an $\epsilon > 0$ that satisfies the above.
Recall that $\unit = \delta/3$ is our unit of imprecision.
Thus, our choice of $\epsilon$ ensures that our grid is fine-grained enough to capture $\tau$
variations of $f$.
%
For proof purposes, we assume $\epsilon < 0.5$, because we are always free to choose a smaller $\epsilon$.
% \zw{I did a literature search but cannot find proper $\epsilon$-nets related to our problem. It appears at slide 52 at Sanjeev Arora's ICML18 talk.
% The paper is https://arxiv.org/pdf/1703.00573.pdf, and the definition-ish statement is in the last paragraph on page 20. I am not sure if that is
% exactly what we need. Wikipedia also listed several definitions of $\epsilon$-nets, which seems to overcomplicate things. I will use the grid for
% now.}



%\todo{say what happens if grid doesn't perfectly align with $C$}
\paragraph{Grid construction}
Consider a standard \emph{grid} of vertices over $C$, where any two neighboring vertices are axis-aligned and of distance $\epsilon$;
we will call this an $\epsilon$-grid. Let $C'\supset C$
be  $C' = \{\bx\in \R^m\mid (x_1\pm \epsilon, \ldots,x_m\pm \epsilon) \in C\}$. That is, we extend $C$ by $\epsilon$ along each dimension.
Formally, to construct an $\epsilon$-grid, 
pick some $\bx \in C$.
Next, let the set of all vertices of the grid be
\[\{ (x_1 + k_1\epsilon,\ldots,x_m+k_m\epsilon) \in C' \mid k_1,\ldots,k_m \in \mathbb{Z}\}\]
%Because $(x_1 + k_1\epsilon,\ldots,x_m+k_m\epsilon) \in C'$,
%and $C' \supset C$, then the grid can cover $C$.

\begin{example}
    Consider \cref{fig:grid_example}.
    It shows a grid over $\R^2$,
    where each vertex is the intersection of a vertical and a horizontal line.
    $\epsilon=1$, because the distance between neighboring vertices is 1.
\end{example}

\paragraph{Boxes in the grid}
We will use $\cell$ to denote a hyperrectangle (box) whose vertices are from the $\epsilon$-grid.\footnote{
    Throughout, a box $\boxm$ refers to an element of the interval domain,
    and a box $\cell$ refers to a hyperrectangle in the $\epsilon$-grid.
}
Let $\cells$ be the set of all such boxes.
Note that, since $C$ is compact, and $C'$ is also compact. Thus, $\cells$ is a finite set of boxes.
%
\begin{example}
    Consider \cref{fig:grid_example_boxes}.
    It shows three example boxes (highlighted) from the set of all boxes $\cells$.
    Note that boxes in $\cells$ may overlap. 
\end{example}
%

We can represent a box $\cell \in \cells$ as 
$[a_1, b_1]\times\ldots\times[a_m, b_m]$,
where 
$[a_i, b_i]$ is the range of the box in dimension $i$. 
%
Because the range is a multiple of $\epsilon$,
$\forall i\ldotp b_i - a_i\geq \epsilon$.
%
Given a box $\cell \in \cells$,
when we say $f(\cell) \geq a$, we mean $\forall \bx \in \cell\cap C \ldotp f(\bx) \geq a$. We use $\cell\cap C$ because $f$
might not be defined outside $C$.


%\todo{fix $G'$ may not be in the grid or $C$}
\paragraph{Neighborhoods}
%Let $C'' = \{\bx\in \R^m\mid (x_1\pm\epsilon, \ldots,x_m\pm k_m\epsilon) \in C'\}$. $C''$ is the extension of $C'$ along each dimension 
%by $\epsilon$.
Let $\cell\in \cells$ and $\cell'$ be a box in $\R^m$.
Then,
$\cell'$ is the \emph{neighborhood} of $\cell$ iff $$\forall i\in\{1,\ldots,m\}\ldotp a_i - a_i' = b_i'-b_i = \epsilon$$
where $[a_i,b_i]$ and $[a_i',b_i']$
are ranges of the $i$th dimension of $\cell$ and $\cell'$, respectively.
% \todo{can't you say: they share a vertex?}
% \zw{yes we can.}
%
%\todo{check the definition dealing with boundaries}
%In other words, $\cell' \in \cells'$ is the tightest box whose boundary is not in $\cell$.
We will use  $\ngbr(\cell)$ denote the neighborhood of $\cell$. 
%Notice that, by definition, $\cell \in \ngbr(\cell)$. 

\begin{example}
Consider \cref{fig:grid_example_box}.
The highlighted 
box is the  neighborhood of the (white) box  $\cell$.
\end{example}


\subsection{Key ideas and indicator functions}\label{sec:step2int}

Our goal is to construct a neural network $\bumpc$
that tells us whether we are in a grid box $\cell$.
This is the most involved construction of the proof.
In this section, we give an intuitive explanation of our methodology.
Then, we proceed to formalize it.

\paragraph{Indicator functions}
%
To tell whether a value $\bx$ is in grid box $\cell$,
we need an \emph{indicator} function,
which, ideally, we can define as follows:
\[\bump_\cell(\bx) = \left\{ \begin{array}{ll}
    1, & \mbox{$\bx \in \cell$}\\
    0, & \mbox{$\bx \not\in \cell$} \end{array} \right.\]
Note how the value is $1$ if $\bx$ is in the box $\cell$,
and $0$ otherwise.



\paragraph{Indicator functions from activation functions}
Our goal is to construct an indicator function from any limit-bounded activation function
satisfying \cref{eq:bounded}.
This is challenging, as such functions are highly unconstrained---essentially, all we know is that they have left and right limits.

Given any limit-bounded activation function $\act$,
a key observation is that if we dilate $\act$ properly, i.e., multiply the input with a large number $\dilate$ to get $\act(\dilate x)$, we will obtain an approximation of the sign (or step)
indicator function---a function that tells whether an input is positive or negative:
%
\[ \step(x) = \left\{ \begin{array}{ll}
    1, & \mbox{$x \geq 0$}\\
    0, & \mbox{$x < 0$}\end{array} \right.\]
 %   

 \begin{example}
    \cref{fig:step_fn} shows the sign indicator function, $\step(x)$.
    \cref{fig:dilated_sigmoid}
    shows a dilated sigmoid function, $\sigma(10x)$,
    approximating the sign function.
 \end{example}


A sign function can be used to construct an indicator function for 1-dimensional boxes.
For example,
\[\step(x) - \step(x-1)\]
returns 1 for $x \in (0,1]$, and 0 otherwise.
%
The following example illustrates that we can approximate 
1-dimensional indicator functions using an activation function.

\begin{example}
    \cref{fig:bump} shows the  box 
    indicator function $\step(x)-\step(x-1)$.
    \cref{fig:dilated_sigmoid_bump} shows the subtraction of two sigmoids,
    $\sigma(10x) - \sigma(10(x-1))$,
    approximating $\step(x)-\step(x-1)$.
\end{example}


In what follows,
we will use the above ideas to approximate
the sign  function and
the indicator function for $m$-dimensional boxes.

\input{ill_step2_bump}

\subsection{Approximating a one-dimensional indicator function}\label{sec:step21d}
We will first show  how to construct an indicator function for a 1-dimensional box, using a limit-bounded activation function.
The main challenge is choosing the dilation factor that results in small precision loss when abstractly
interpreting the neural network.

By the AUA theorem statement, we are given some limit-bounded
activation function $\act$. 
Without loss of generality, we make the following two assumptions
about $\act$:
\begin{enumerate}
\item We assume that $\act$ already satisfies \cref{eq:bounded} (\cref{def:activation}): 
\[ 
    \lim_{x\rightarrow -\infty} \act(x) = a
   \quad  \text{ and } \quad
    \lim_{x\rightarrow \infty} \act(x) = b
    \quad \text{ and } \quad
    \forall x\in \R\ldotp \act(x)\in[a, b]
    \]
Otherwise, by \cref{def:activation},
we can use $\act$ to build a $\act'$ that satisfies \cref{eq:bounded}. 

\item We assume that the left and right limits of $\act$ are $0$ and $1$,
respectively.
(If not, we can apply an affine transformation to the results of $\act$
to make the left and right limits $0$ and $1$.)
\end{enumerate}
% %
% Because the activation function is limit-bounded, it has limits at both sides, but the function might not reach the limit value, we are only able to bound the function's range at both sides.
% Therefore, we are only able to create an approximate bump function, and this could lead to loss of precision. Therefore, we need to carefully construct the bump function so that the loss 
% of precision is still within $\delta$ as in~\cref{thm:main}.

% We now give a rigorous treatment of the approximation. 

\paragraph{Loss of precision from limits}
The activation function $\act$ has limits at both sides, but the function might never reach the limit. For example, the right limit of the sigmoid function, $\sigmoid$, is $1$, but $\forall x\ldotp\sigmoid(x) \neq 1$.
This will lead to a loss of precision when we use $\act$  to model a sign function. 
However, because $\act$ has limits, we can bound the range of $\act$ around its limit. By properly 
bounding the range, we can ensure that the loss of precision is within the tolerated amount.


Recall that $K+1$ is the number of slices of $f$.  
The final step of the proof sums over all
function-slice approximations, and we would like to control precision loss caused by the limit behavior of $\act$ to be within $\unit$.
Because each function-slice approximation can lose at most $\unit$ precision, 
we choose the precision loss from $\act$ to be $\lprec \leq \frac{1}{K+1}$.
Therefore,
$(K+1)\lprec \unit\leq \unit$.
%\todo{this paragraph is somewhat confusing, we want to control precision loss within $0.5\tau$, but then $\theta$ says nothing about $\tau$.}
%\aws{< or $\leq$?}
%Our construction of the neural network 
%$\nn_i$, which approximates slice $f_i$, will be the sum over bump functions 
%for potentially all cells in $C$, and the final neural network is a sum of all $\nn_i$ for $i\in \{0, 1,\ldots, K\}$, a total of $K+1$ slices. All slices can introduce 
%$(K+1)|\cells|$ units of imprecision. Define $V = 2(K+1)|\cells|$
%\footnote{\aws{we should remove this footnote}\label{ft:V}We can choose any $V$ as we want, because it is also used in the analysis in~\cref{lem:cell}, without 
%loss of generality, we can assume $V = 2(K+1)|\cells| \geq 4m+2$; otherwise, let $V = \max(2(K+1)|\cells|, 4m+2)$.}, 
%and let $\lprec$ be the precision loss for a single bump function.
%Then the imprecision introduced from the limit behavior rather than exact values of all the activation function is 
%restricted to $(K+1)|\cells|\times (\lprec) = 0.5$ unit in the final precision analysis.
%\aws{what does limit behavior rather than exact values mean?}


% \begin{proof}
%     In the definition of limit, let $\xi = \lprec$. Then $\exists D$ such that if $x>D$, $|\act(x)-1| < \lprec$; and if $x>D$, $|\act(x)-0| < \lprec$.

%     $|\act(x)-1| < \lprec \iff 1-\lprec<\act(x)<1+\lprec$; $|\act(x)-0| < \lprec \iff -\lprec < \act(x)< \lprec$.

%     Also because $\forall x\ldotp 0\leq \act(x)\leq 1$ (see~\cref{eq:bounded}), then if $x> D$, $1-\lprec<\act(x)\leq 1$; and if $x< -D$, $0\leq\act(x)<\lprec$.
% \end{proof}


\paragraph{Dilation to approximate sign function}
%
We now discuss how to dilate $\act$ to get a sign-function-like behavior.
By definition of limit, we know the following lemma,
which states that by sufficiently increasing the input of $\act$, we can get $\lprec$ close to the right limit of $1$,
and analogously for the left limit.
\begin{lemma}\label{lem:limit}
    $\exists D > 0$ such that:
    \begin{enumerate}
    \item If $x\geq D$, then $\act(x)\in (1-\lprec, 1]$.
    \item If $x\leq -D$, then $\act(x)\in[0,\lprec)$.
    \end{enumerate}
\end{lemma}

Because the grid size is $\epsilon$, we want the sign-function approximation to achieve a transition from  $\approx 0$ to  $\approx 1$ within $\epsilon$. Let $\dilate$ be the \emph{dilation factor}.
Following \cref{lem:limit}, we would like the following: 
\begin{enumerate}
    \item if $x\geq 0.5\epsilon$, then $\act(\dilate x)\in (1-\lprec, 1]$; 
    \item if $x\leq -0.5\epsilon$, then $\act(\dilate x)\in[0,\lprec)$.
\end{enumerate}

From~\cref{lem:limit}, we only need $\dilate x > D$ when $x> 0.5\epsilon$; therefore, $\dilate = 2D/\epsilon$ suffices as the dilation factor.

\begin{lemma}\label{lem:dilate}
    Let $\dilate = 2D/\epsilon$. The following is true:
    \begin{enumerate}
        \item if $x\geq 0.5\epsilon$, then $\act(\dilate x)\in (1-\lprec, 1]$; 
        \item if $x\leq -0.5\epsilon$, then $\act(\dilate x)\in[0,\lprec)$.
    \end{enumerate}
\end{lemma}

\begin{example}
    \cref{fig:loss_step}
    illustrates the loss of precision $\lprec$
    incurred by our construction.
\end{example}

\begin{wrapfigure}{r}{0.4\textwidth}
    \vspace{-1em}
    \centering
    \begin{tikzpicture}
      \begin{axis}[
        axis lines=middle,
        xmax=4,
        xmin=-4,
        ymin=-0.15,
        ymax=1.1,
        ytick={0,1},
        xtick={0},
        width=4.7cm
    ]
  
    \addplot [domain=-5:5, samples=100, thick, blue] {1/(1+exp(-x))};
    \draw [dotted] (1,0) -- (1,1);
    \draw [dotted] (-1,0) -- (-1,1);
    \draw [dotted] (-10,1) -- (10,1);
    \draw[<->,red] (1,1) -- (1,0.73);
    \draw[<->,red] (-1,0) -- (-1,0.27);
    \node at (0.5,0.85) {\footnotesize$\leq\lprec$};
    \node at (1,-.1) {\footnotesize$0.5\epsilon$};
    \node at (-1,-.1) {\footnotesize$-0.5\epsilon$};

  \end{axis}
    \end{tikzpicture}
    \vspace{-1em}
    \caption{Illustrating the loss of precision $\lprec$ incurred through using a limit-bounded activation to approximate a sign function.
    The length of the red arrows is $\leq \lprec$.}
    \label{fig:loss_step}
\end{wrapfigure}

\paragraph{Indicator function on dimension $i$}
Now that we have discussed how to approximate
a sign function, we are ready to show
how to approximate an indicator function
for one dimension of a box $\cell$ in the grid.

Suppose the projection of a box $\cell$ on dimension $i$ is $[a_i, b_i]$. 
Because $\cell$ is in the $\epsilon$-grid, $b_i-a_i\geq \epsilon$; and the projection of neighborhood $\ngbr(\cell)$ on 
dimension $i$ is $[a_i-\epsilon, b_i+\epsilon]$. We want to build an indicator function that has value close to $1$ on $[a_i, b_i]$, and value close to $0$ on 
$\R\setminus [a_i-\epsilon, b_i+\epsilon]$. 
Notice how we may lose precision within the
neighborhood of $\cell$;
this is expected, because our approximation may not be able
to exactly tell if we are in $\cell$ or its neighborhood.

Inspired by how to construct an indicator function from a sign function, we will take the difference between two shifted step functions. Let
\begin{equation}
\bumpi(x) = \act\left(\dilate\left(x+0.5\epsilon - a_i\right)\right) -\act\left(\dilate\left(x-0.5\epsilon - b_i\right)\right)
\end{equation} 


\paragraph{Properties of $\bumpi$}
The following lemmas show that $\bumpi$ roughly behaves like an indicator function:
its value within a box's $i$th dimension $[a_i,b_i]$
is $\approx 1$;  
its value outside of the neighborhood is $\approx 0$;
its value globally is bounded by $1$
%
We will analyze the values of the two terms in $\bumpi$.

The following lemma states
that if $x$ is within the box's $i$th dimension,
then the first term is close to 1 and the second term is close to 0,
resulting in $\bumpi(x) \approx 1$.

%\aws{interval notation}

\begin{lemma}\label{lem:step_1}
    If $x\in [a_i, b_i]$, then the following is true:
    \begin{enumerate}
    \item $\act(\dilate(x+0.5\epsilon - a_i))\in(1-\lprec, 1]$.
    \item $\act(\dilate(x-0.5\epsilon- b_i))\in[0, \lprec)$.
    \end{enumerate}
\end{lemma}

% \begin{proof}
%     \textbf{Point (1):} 
%         Because $x\geq a_i$, $x+\epsilon/2 - a_i \geq \epsilon/2$, from~\cref{lem:dilate}, $1-\lprec<\act(\dilate(x+\epsilon/2 - a_i))\leq 1$.

%     \textbf{Point (2):}
%         Because $x\leq b_i$, $x-\epsilon/2 - b_i\leq -\epsilon/2$, from~\cref{lem:dilate}, $0\leq \act(\dilate(x-\epsilon/2 - b_i))< \lprec$.
% \end{proof}

The next two lemmas state that if $x$ is outside the neighborhood,
then the two terms are similar, resulting in a $\bumpi(x) \approx 0$.

\begin{lemma}\label{lem:step_2}
    If $x\leq a_i-\epsilon$, then the following is true:
    \begin{enumerate}
    \item $\act(\dilate(x+0.5\epsilon - a_i))\in[0, \lprec)$.
    \item $\act(\dilate(x-0.5\epsilon- b_i))\in[0, \lprec)$.
    \end{enumerate}
\end{lemma}


\begin{lemma}\label{lem:step_3}
    If $x\geq b_i+\epsilon$, then the following is true:
    \begin{enumerate}
    \item $\act(\dilate(x+0.5\epsilon - a_i))\in(1-\lprec, 1]$.
    \item $\act(\dilate(x-0.5\epsilon - b_i))\in(1-\lprec, 1]$.
    \end{enumerate}
\end{lemma}


\paragraph{Abstract precision of $\bumpi$}
We are now ready to prove properties about the abstract interpretation
of our 1-dimensional indicator approximation, $\bumpi$.
The following lemma states that the abstract interpretation
of $\bumpi$, $\absbumpi(\boxm)$, is quite precise:
if the 1-dimensional input box $\boxm$ is outside the neighborhood of $\cell$,
on $\cell$'s $i$th dimension,
then the output box is within $\lprec$ from 0;
if the input box $\boxm$ is within the $i$th dimension of $\cell$,
then the output box is within $2\lprec$ from 1. 

\begin{lemma}\label{lem:abs_single_bump}
    For a 1-dimensional box $\boxm$, the following is true:
    \begin{enumerate}
    \item $\bumpi^\#(\boxm) \subset (-\infty, 1]$.
    \item If $\boxm \subseteq (-\infty, a_i-\epsilon]$ or $\boxm\subseteq [b_i+\epsilon, \infty)$, then $\bumpi^\#(\boxm)\subseteq (-\lprec, \lprec)$.
    \item If $\boxm \subseteq [a_i, b_i]$, then $\bumpi^\#(\boxm)\subseteq (1-2\lprec, 1]$ .
    \end{enumerate}
\end{lemma}
\begin{proof}
    %\zw{change $l, u$ to $a, b$?}
    %\aws{sure}
    We begin the proof by simplifying the expression $\absbumpi(\boxm)$.
    Recall that $\bumpi(x) = \act(\dilate(x+0.5\epsilon - a_i)) -\act(\dilate(x-0.5\epsilon - b_i))$.
    Let $\boxm = \langle[a,b]\rangle$.
    By applying abstract transformer $\absact$ (\cref{def:abstrans}) and subtracting the two terms,
    we get $\absbumpi(\boxm) = [T_1-T_4, T_2-T_3]$,
    where 

% \[
%     \begin{array}{lllr}
%         \absbumpi(\boxm) &=& \absact(\dilate^\#\abstimes(\boxm\absplus(\epsilon/2)^\#\absplus -(a_i)^\#)) \absplus -\absact(\dilate^\#\abstimes(\boxm\absplus -(\epsilon/2)^\# \absplus -(b_i)^\#))& \\
%          && \hfill\mbox{(apply abstract transformers)} & \\
%                    &=& \absact(\dilate^\#\abstimes([a, b]\absplus(\epsilon/2)^\#\absplus -(a_i)^\#)) \absplus -\absact(\dilate^\#\abstimes([a, b]\absplus -(\epsilon/2)^\# \absplus -(b_i)^\#) &\\
%         && \hfill \mbox{(expand $\boxm$)} & \\
%                    &=& \absact([\dilate(a+\epsilon/2-a_i), \dilate(b+\epsilon/2-a_i)]) \absplus - \absact([\dilate(a - \epsilon/2 -b_i), \dilate(b - \epsilon/2 -b_i)])  & \\
%                    && \hfill\mbox{(expand arguments of $\absact$)} &  \\
%     \end{array}
%     \]
%     %
%     Following the definition of the abstract transformer, $\absact$,
%     let 
    \[
        \begin{array}{lll}
        T_1 = \min_{x\in[a,b]}\act(\dilate(x+0.5\epsilon-a_i)) &&
        T_2 = \max_{x\in[a,b]}\act(\dilate(x+0.5\epsilon-a_i))\\
        T_3 = \min_{x\in[a,b]}\act(\dilate(x-0.5\epsilon-b_i)) &&
        T_4  = \max_{x\in[a,b]}\act(\dilate(x-0.5\epsilon-b_i))
        \end{array}
    \]
    % Then,

    % \begin{equation}\label{eq:abs_bumpi}
    %     \begin{array}{lllr}
    %         \absbumpi(\boxm) &=& [T_1, T_2]\absplus -[T_3, T_4] & \mbox{(definition of $\absact$)}\\
    %                      &=& [T_1, T_2]\absplus [-T_4, -T_3] & \mbox{(multiply by $-1$)}\\
    %                      &=& [T_1-T_4, T_2-T_3] & \mbox{(apply $\absplus$)}\\
    %     \end{array} 
    % \end{equation}
    
    We are now ready to prove the three statements.

    \vspace{0.5em}\noindent
    \textsc{Statement (1):}
    By  limit-boundedness of $\act$, $\forall x\ldotp \act(x)\in [0,1]$, so $T_1, T_2, T_3, T_4\in [0, 1]$. 
    Therefore, the upper bound of $\absbumpi(\boxm)$ is $T_2 - T_3\leq  1$.


    \vspace{0.5em}\noindent
    \textsc{Statement (2):}

    \begin{mycases}
    \case $\boxm \subseteq (-\infty, a_i-\epsilon]$. 
    %$a, b\in (-\infty, a_i-\epsilon]$. 
    From~\cref{lem:step_2}, 
    $T_1, T_2, T_3, T_4\in [0, \lprec)$, then $T_2-T_3 < \lprec$, and $T_1-T_4 > -\lprec$.
    
    \case $\boxm \subseteq [b_i+\epsilon, \infty)$. 
    %$a, b\in (-\infty, a_i-\epsilon]$. 
    From~\cref{lem:step_3}, 
    $T_1, T_2, T_3, T_4\in (1-\lprec, 1]$, then $T_2-T_3 < \lprec$, and $T_1-T_4 > -\lprec$.

    \end{mycases}
    In either case, $\bumpi^\#(\boxm)\subseteq (-\lprec, \lprec)$.

    \vspace{0.5em}\noindent
    \textsc{Statement (3):}
%
    If $\boxm \subseteq [a_i, b_i]$, $a, b\in [a_i, b_i]$. From~\cref{lem:step_1}(1), 
    $T_1, T_2\in (1-\lprec, 1]$. From~\cref{lem:step_1}(2), $T_3, T_4\in [0, \lprec)$. 
    Then $T_1-T_4 > 1-2\lprec$ and $T_2-T_3\leq 1$.

    Therefore, $\bumpi^\#(\boxm)\subseteq (1-2\lprec, 1]$.
\end{proof}


%\begin{lemma}[Properties of 1-dimensional bump approximation, $\bumpi$]\label{lem:single_bump}
%    The following is true:
%    \begin{enumerate}
%    \item If $a_i\leq x\leq b_i$, then $1-2\lprec<\bumpi(x)\leq 1$ .
%    \item If $x\leq a_i-\epsilon$ or $x\geq b_i+\epsilon$, then $-\lprec<\bumpi(x)<\lprec$.
%    \item $\forall x\in \R \ldotp \bumpi(x) \leq 1$.
%    \end{enumerate}
%\end{lemma}


%\aws{this point uses $x_i$, but we should use $x$}
%\aws{also same complaint as above}
%\textbf{Point (2):} Either $x_i\leq a_i-\epsilon$ or $x_i\geq b_i+\epsilon$:
%\begin{mycases}
%    \case If $x_i\leq a_i-\epsilon$, 
%        \subcase $x+\epsilon/2 - a_i\leq -1/2\epsilon$, from the choice of $\dilate$, $0\leq \act(\dilate(x+\epsilon/2 - a_i))< \lprec$;
%        \subcase $x-\epsilon/2 - b_i\leq -5/2\epsilon$, from the choice of $\dilate$, $0\leq \act(\dilate(x-\epsilon/2 - b_i))< \lprec$.
    
%    Therefore, $-\lprec < \act(\dilate(x+\epsilon/2 - a_i)) -\act(\dilate(x-\epsilon/2 - b_i))< \lprec$.

%    \case If $x_i\geq b_i+\epsilon$, 
%        \subcase $x+\epsilon/2 - a_i\geq 5/2\epsilon$, from the choice of $\dilate$, $1-\lprec< \act(\dilate(x+\epsilon/2 - a_i))\leq 1$;
%        \subcase $x-\epsilon/2 - b_i\geq 1/2\epsilon$, from the choice of $\dilate$, $1-\lprec< \act(\dilate(x-\epsilon/2 - b_i))\leq 1$.
   
%    Then $-\lprec < \act(\dilate(x+\epsilon/2 - a_i)) -\act(\dilate(x-\epsilon/2 - b_i))< \lprec$.
%\end{mycases}
%In either case, $-\lprec < \act(\dilate(x+\epsilon/2 - a_i)) -\act(\dilate(x-\epsilon/2 - b_i))< \lprec$.\\



%\textbf{Point (3):} 
%    Because $\act(x) \in [0,1]$ for any $x$, then $\act(x) - \act(y)\leq 1$ always hold for any $x, y\in \R$. Then 
%    $\bumpi(x) = \act(\dilate(x+\epsilon/2 - a_i)) -\act(\dilate(x-\epsilon/2 - b_i))\leq 1$.
%\end{proof}

% From~\cref{lem:single_bump}, we have built the bump function on dimension $i$.


%\paragraph{Remark} Technically we can design any integer rather than use $A$ in~\cref{eq:bump}, but $A$ is sufficient for our need.

\begin{figure}

    \begin{subfigure}{.4\textwidth}
        \begin{center}
            \begin{tikzpicture}
                % nodes
                \draw node at (0, 0) [input] (in) {$x_1$};
                \draw node at (0, -2) [input] (in2) {$x_m$};
                \draw node at (0, -.9) [input] (dots) {$\vdots$};
        
                \draw node at (1, 0) [oper] (plus) {$\bumpi_1$};
                \draw node at (1, -.9) [input] (dots) {$\vdots$};
        
        
        
                \draw node at (1, -2) [oper] (plus1) {$\bumpi_m$};
                
        
                \draw node at (2, -1) [oper] (sum) {$\sum$};
                \draw node at (3.5, -1) [oper] (act) {$\act$};
        
                \draw[->,thick] (in) -- (plus);
                \draw[->,thick] (in2) -- (plus1);
                \draw[->,thick] (plus) -- (sum);
                \draw[->,thick] (plus1) -- (sum);
                \draw[->,thick] (sum) to node[above]{$\dilate$} (act);
                \draw[->,thick] (act) -- (4,-1);            
            \end{tikzpicture}
        \end{center}
        \caption{\footnotesize Illustration of $\bumpc$ (added constants elided)}
        \label{fig:nng}
        \end{subfigure}
%
\quad
    \begin{subfigure}{.55\textwidth}

    \centering
    \begin{tikzpicture}
        \begin{axis}[grid=both,restrict z to domain=0:1,width=4cm]
            \addplot3 [surf] {1/(1+exp(-10 * (1/(1+exp(-10*(x+1/2))) - 1/(1+exp(-10*(x-1.5))) + 1/(1+exp(-10*(y+0.5))) - 1/(1+exp(-10*(y-1.5))) -0.90 - 0.95 )))};
          \end{axis}
    \end{tikzpicture}
    \caption{\footnotesize Plot of $\bumpc$ on $\cell =  [0,1] \times [0,1]$
    using the sigmoid activation, with $\dilate=10$, $2\lprec = 0.05$, and $\epsilon=1$.
    Observe how  $\bumpc(\bx)$ is $\approx 1$ for values of $\bx \in \cell$,
    and $\approx 0$ elsewhere.}\label{fig:2d}
\end{subfigure}
\caption{\textbf{Step 2} Illustration of neural network $\bumpc$}
\end{figure}

\subsection{Approximating an $m$-dimensional indicator}\label{sec:step2md}

%\paragraph{Constructing cell approximation}
We saw how to construct an indicator approximation for a 1-dimensional box.
We will now show how to construct an indicator function approximation $\nn_\cell$
for an $m$-dimensional box.

Throughout, we assume a box $\cell = [a_1,b_1]\times \cdots \times [a_m,b_m]$.
So, if $\bx\in \cell$, then $x_i\in[a_i, b_i]$ for all $i \in \{1,\ldots,m\}$; 
if $\bx \not\in \ngbr(\cell)$, i.e., not in the neighborhood, 
then $\exists i$ such that
$x_i\leq a_i-\epsilon$ or $x_i\geq b_i+\epsilon$. 


\paragraph{Constructing $\bumpc$}
We want to construct an indicator function whose value within a box $\cell$ is close to $1$ and outside the neighborhood $\ngbr(\cell)$ is close to $0$.
 In the multi-dimensional case, $m\geq 2$,  we do 
 not know at which, if any, dimension $j$ of an input is outside the neighborhood of $\cell$. 
 The 1-dimensional indicator approximation, $\bumpi$, 
 which we constructed earlier, can be used to tell us, for each dimension $j$,
 whether $x_j$ is within the bounds of the neighborhood of $\cell$.
 Therefore we can construct a logical OR
 approximation that applies $\bumpi$
 to each dimension and takes the OR of the results.
Specifically,
 \begin{enumerate}
 \item
 We will construct a function that applies $\bumpi$ to each dimension,
 and sums the results such that the answer is $>0$ if $\bx \in \cell$,
 and $< 0$ if $\bx \not\in \ngbr(\cell)$.
 \item Then, we can use the sign-function approximation to 
  indicate the sign of the answer.
 \end{enumerate}
  %
 Formally, we define the neural network $\nn_\cell$ as follows:
% We want to construct a bump function where the value within the a cell $\cell$ is close to $1$ and outside the immediate neighbors close to $0$.
% The challenge with the multi-dimensional case, $m\geq 2$, is that we do 
% not know at which dimension $j$, $x_j\in\R\setminus [a_j-\epsilon, b_j+\epsilon]$. Therefore, we will treat all dimensions symmetrically. Specifically, 
% We will use a function $\sum_{i=1}^m H_i$ to handle that at some dimension $j$, $x_j$ is out of range of $\ngbr(G)$.
% \aws{the last sentence doesn't make sense. We start by saying we don't know what dimension is out of the ngbrhood, but then say we're going to create a function $H_i$ for each dimension... how is that a solution?}
% \zw{The point is if we have a function for each dimension, then we take its sum to handle the issue that we do not know which dimension is out of range.}

% \aws{this next paragraph also doesn't make sense: which $\act$ are we talking about?}\zw{See the text above, the two usages of step function.}
% Because we have dilated $\act(x)$ to approximate a step function, this can help build the multi-dimensional bump function. When $\bx\in \cell$, the input to 
% $\act$ is in the positive piece of the step function, and when $\bx\in C\setminus \ngbr(G)$, the input to $\act$ is in the $0$ piece of the step function. Therefore, 
% we will build the multi-dimensional bump function $\bumpc$ in the following form:


\begin{equation}\label{eq:bump}
    \bumpc(\bx) = \act\left(\dilate\left(\sum_{i=1}^m H_i(x_i)+0.5\epsilon\right) \right)
\end{equation}
where $H_i(x) = \bumpi_i(x) - (1- 2\lprec)$,
and $\bumpi_i$ is $\bumpi $ using the range $[a_i,b_i]$ of the $i$th dimension of $\cell$.
%
The neural network $\bumpc$ is graphically depicted in \cref{fig:nng}.

The function term $\sum_{i=1}^m H_i(x_i)$ evaluates to a positive
 value if $\bx \in \cell$ and to a negative value if $\bx \not\in \ngbr(\cell)$.
 Observe that we need to shift the result of $\bumpi$ by $(1-2\lprec)$
 to ensure a negative answer if one of the dimensions is outside the neighborhood.
 %
 Then, we use $\act$ to approximate the sign function, as we did in the 1-dimensional case, 
 giving $\approx1$
 if $\bx \in \cell$, and $\approx0$ if $\bx \not\in \ngbr(\cell)$.

\begin{example}
\cref{fig:2d} shows a plot of $\bumpc$
for $\bx \in \R^2$.
\end{example}

\paragraph{Abstract precision of $\nn_\cell$}
We are now ready to analyze the abstract precision of $\nn_\cell$.
We first consider $H_i$ in the following lemma.
For any box $B\subseteq C$, let $B_i$ be its projection on dimension $i$, which is an interval.

The following lemma states that if $\boxm$ is in the box $\cell$,
then $\sum_i H_i^\#$ is positive; otherwise, if $\boxm$ is outside
the neighborhood of $\cell$, then $\sum_i H_i^\#$  is negative.

\begin{lemma}[Abstract interpretation of $H_i$]\label{lem:abs_cell}
    For any box $B\subseteq C$, the following is true:
    \begin{enumerate}
        \item If $B\subseteq \cell$, then $\sum_{i=1}^mH_i^\#(B_i) \subseteq (0, \infty)$.
        \item If $B\subseteq C\setminus\nu(\cell)$, then $\sum_{i=1}^mH_i^\#(B_i) \subseteq (-\infty, -\epsilon)$.
    \end{enumerate}
\end{lemma}

The following theorem states the precision of the abstract interpretation of $\bumpc$:
if the input box is in $\cell$,
then the output box is within $\theta$ from $1$;
if $\boxm$ is outside the neighborhood of $\cell$,
then the output box is within $\theta$ from $0$.

%\begin{lemma}[Properties of $H_i$]\label{lem:cell}
%    The following is true:
%    \begin{enumerate}
%        \item If $\bx\in \cell$, then $\sum_i^mH_i(x_i) > 0$.
%        \item If $\bx\in C\setminus\ngbr(\cell)$, then $\sum_i^mH_i(x_i) < -\epsilon$.
%    \end{enumerate}
%\end{lemma}
%\begin{proof}
%    \textbf{Point (1):}
%    If $a_i\leq x_i\leq b_i$, from~\cref{lem:single_bump}, $\bumpi_i(x) > 1-2\lprec$, so $H_i(x) > 0$. Thus, if $\bx\in \cell$, then $\forall i\in\{1,\ldots, m\}$,
%    $a_i\leq x_i \leq b_i$, so $\sum_{i=1}^mH_i(x_i) > \sum_{i=1}^m 0 = 0$.\\
    
%    \textbf{Point (2):}  If $\bx\in C\setminus\ngbr(\cell)$ ,then $\exists j$ such that $x_j\leq a_j-\epsilon$ or $x_j\geq b_j+\epsilon$, 
%    by~\cref{lem:single_bump}, $\bumpi_j(x)< \lprec$, and  \[H_j(x) = \bumpi_i(x) - (1-2\lprec) < \lprec-(1-2\lprec) = 3\lprec-1.\]

%    For the remaining $m-1$ dimensions, because $\bumpi_i(x_i) \leq 1$ is always true (\cref{lem:single_bump}), then $H_i(x) = \bumpi_i(x_i) - (1-2\lprec)\leq 2\lprec$ when $i\neq j$.
%    Hence, $\sum_{i\in \{1,\ldots,m\}\setminus{j}}H_i(x)\leq \sum_{i\in \{1,\ldots,m\}\setminus{j}}2\lprec = 2(m-1)\lprec$. 
    
%    Sum over all the $m$ dimensions we have $\sum_{i=1}^m H_i(x_i) = \sum_{i\in \{1,\ldots,m\}\setminus{j}}H_i(x) + H_j(x) < 2(m-1)\lprec + 3\lprec - 1 = (2m+1)\lprec - 1$. 
%    Because we assume $V \geq 4m+2$ (see~\cref{ft:V}), then $\sum_{i=1}^m H_i(x_i)\leq(2m+1)/(4m+2) - 1 = 1/2 - 1 = -1/2$. Also we assume that $\epsilon < 1/2$ (see~\cref{ft:eps}), 
%    then $\sum_{i=1}^m H_i(x_i)\leq -1/2 < -\epsilon$.
%\end{proof}


%\begin{theorem}[Properties of $\bumpc$]\label{thm:bump}
%    The following is true:
%    \begin{enumerate}
%        \item $\forall \bx \in C$, $\bumpc(\bx)\in [0, 1]$.
%        \item If $\bx \in \cell$, $\bumpc(\bx)\in (1-\lprec, 1]$.
%        \item If $\bx \in C\setminus\ngbr(\cell)$, $\bumpc(\bx)\in [0, \lprec)$.
%    \end{enumerate}
%\end{theorem}

%\begin{proof}
%    \textbf{Point (1):}
%    See~\cref{eq:bump}, because outer function of $\bumpc$ is $\act$, whose range is $[0,1]$ by the definition of limit-boundness.

%    \textbf{Point (2):}
%    If $\bx \in \cell$, from~\cref{lem:cell}, $\sum_i^mH_i(x_i)+\epsilon/2 > 0 + \epsilon/2 > \epsilon/2$. Because of the choice of the dilation factor $\dilate$, 
%    $\bumpc(\bx) = \act(\dilate(\sum_{i=1}^mH_i(x_i)+\epsilon/2))\in (1-\lprec, 1]$.

%    \textbf{Point (3):}
%    If $\bx \in C\setminus\ngbr(\cell)$, from~\cref{lem:cell}, $\sum_i^mH_i(x_i)+\epsilon/2 < -\epsilon + \epsilon/2 = -\epsilon/2$. Because of the choice of the dilation factor $\dilate$, 
%    $\bumpc(\bx) = \act(\dilate(\sum_{i=1}^mH_i(x_i)+\epsilon/2))\in [0, \lprec)$.
%\end{proof}

\begin{theorem}[Abstract interpretation of $\bumpc$]\label{thm:abs_bump}
    For any box $B \subseteq C$, the following is true:
    \begin{enumerate}
        \item $\absbumpc(B)\subseteq [0, 1]$.
        \item If $B\subseteq \cell$, then $\absbumpc(B)\subseteq (1-\lprec, 1]$.
        \item If $B\subseteq  C\setminus\ngbr(\cell)$,  then $\absbumpc(B)\subseteq [0, \lprec)$.
    \end{enumerate}
\end{theorem}

\begin{proof}
~\\\noindent
\textsc{Statement (1):}
%
See definition of $\bumpc$ in ~\cref{eq:bump}. 
The outer function of $\bumpc$ is $\act$, whose range is $[0,1]$ by the definition of limit-boundedness and our assumption that the left and right limits are $0$ and $1$.
Therefore, $\absbumpc(B)\subseteq [0, 1]$.

\vspace{0.5em}\noindent
\textsc{Statement (2):}
%
If $\boxm \subseteq \cell$, from~\cref{lem:abs_cell}, 
we know that $\sum_{i=1}^mH_i^\#(B_i) \subseteq (0, \infty)$.
Then,
\[
\sum_i^mH_i^\#(\boxm_i)\absplus (0.5\epsilon)^\# 
\quad \subseteq \quad
(0, \infty) \absplus (0.5\epsilon)^\# \\ 
\quad \subseteq \quad  (0.5\epsilon, \infty)
\] 
%\zw{Minor, should we change the last $\subseteq$ to $=$? and similarly for the statement 3.}
%\aws{it doesn't matter}
From~\cref{lem:dilate}, 
we know that if $x\geq 0.5\epsilon$, then $1-\lprec<\act(\dilate x)\leq 1$.
Therefore,
\[
\absbumpc(\boxm) = \absact(\dilate^\# \abstimes (0.5\epsilon, \infty))
\quad  \subseteq \quad  (1-\lprec, 1]
\]

\noindent
\textsc{Statement (3):}
%
If $B\subseteq C\setminus\nu(\cell)$, from~\cref{lem:abs_cell}, 
we know that $\sum_{i=1}^mH_i^\#(B_i) \subseteq (-\infty, -\epsilon)$. 
Then, \[
\begin{array}{lll}
\sum_{i=1}^m H_i^\#(B_i) \absplus (0.5\epsilon)^\# \quad \subseteq \quad
(-\infty,-\epsilon) \absplus (0.5\epsilon)^\#
\quad \subseteq \quad  (-\infty, -0.5\epsilon)
\end{array}
\] 
From~\cref{lem:dilate}, 
we know that if $x\leq -0.5\epsilon$, then $0\leq\act(\dilate x)<\lprec$.
Therefore,
\[
    \absbumpc(\boxm)  =  \absact(\dilate^\# \abstimes (-\infty, -0.5\epsilon))
    \quad \subseteq \quad  [0, \lprec)
\]
\end{proof}


% \paragraph{Step activation function}
% % The grid forms a partition of $C$, and we will define a step function on the grid to approximate $f_i$. If we revisit the definition of $f_i$, we can
% % see that the input space is partitioned into three parts: $\{x\in C| f(x) \leq i\delta/3\}$,  $\{x\in C| f(x) \geq (i+1)\delta/3\}$ and  
% % $\{x\in C| i\delta/3<f(x) < (i+1)\delta/3\}$. We will find the grid approximation of the three parts.
% %
% % Fix $k$, define $U_k = \{g\in G| f(g) \geq (k+1)\delta/3\}$; and $L_k=\{g\in G| f(g) \leq k\delta/3\}$. 
% % Let $S_k = \cup_{(g\in U_k)} g$, and $\bar{S}_k =  \cup_{(g\in L_k)} g$.
% %
% For every grid cell $\cell \in \cells$, we will approximate it using a step activation function 
% of the form:
% \[
% \act_{\cell}(\bx) = \left\{ \begin{array}{ll}
%     \delta/3  & \bx \in \cell\\
%     0, & \mbox{otherwise}
% \end{array} \right.
% \]
% that is parameterized by cell $\cell$ and a constant $a\in \R$.

% A sound abstract transformer for this activation function is the following:
% \[
% \act^\#_{\cell}(\boxm) = \left\{ \begin{array}{ll}
%     ~[\delta/3,\delta/3]  & \boxm \subseteq \cell\\
%     ~[0,\delta/3], & \mbox{otherwise}
% \end{array} \right.
% \]
% Note that a cell $\cell$ is also a box, and therefore we can check subset inclusion.

% % \aws{what happens at the borders between cells?}
% % \zw{If we use this step function definition, we probably only consider two cases; i.e., without the $\delta/6$ ones to simplify the border.}

% \paragraph{Slice approximation}
% Now, to approximate a slice $f_k$,
% we will need to consider the following set of grid cells:
%  All cells whose values are \emph{above} the $k$th slice
%     (recall that the $k$th slice is the $[k\delta/3, (k+1)\delta/3]$):
%     \[U_k = \{\cell \in \cells \mid f(\cell) \geq (k+1)\delta/3\}\]
%     % \item All cells whose values are \emph{within} the $k$th slice:
%     % \[W_k=\{\cell\in \cells \mid  k \delta/3 \leq f(\cell) \leq (k+1)\delta/3\}\] \zw{This is not accurate.}

% % Fix $k$, define $U_k = \{g\in G| f(g) \geq (k+1)\delta/3\}$; and $L_k=\{g\in G| f(g) \leq k\delta/3\}$. 
% % Let $S_k = \cup_{(g\in U_k)} g$, and $\bar{S}_k =  \cup_{(g\in L_k)} g$.

% We now construct a neural network $\nn_k$ to approximate $f_k$
% as follows:

% % \[ n_k(x) = \left\{ \begin{array}{ll}
% %     0, & \mbox{$x \in \bar{S}_k$}\\
% %     \delta/3, & \mbox{$x \in S_k$}\\
% %     \delta/6, & \mbox{$x \in C\setminus (S_k\cup \bar{S}_k)$} \end{array} \right. \]

% \[
% \nn_k(\bx) = \sum_{\cell \in U_k} \act_{\cell}(\bx)
% % \quad + \quad 
% % \underbrace{\sum_{\cell\in W_k} \act_{\cell,\frac{\delta}{6}}(\bx)}_\text{within $k$th slice}    
% \]

% Recall that the upper bound of the range of $f_k$ is $\delta/3$.
% Therefore, our definition assigns $\nn_k(\bx) = \delta/3$
% for any value of $\bx$ that belongs to a grid cell above the $k$th  slice.
% % If $f(\bx)$ is within the $k$th slice, we set $ \nn_k(\bx) = \delta/6$;\footnote{
% %     In our construction, we can assign any values between $0$ and $\delta/3$ for as the parameter of the second activation function. We choose $\delta/6$ in our construction.
% % }
% if $f(\bx)$ is below or within the $k$th slice, then we set $\nn_k(\bx) = 0$.



% \begin{example}
% Figure~\ref{fig:step} shows $\nn_3$, which approximates $f_3$.
% \end{example}



% \paragraph{Bounding approximation precision loss}
% We will now prove a lemma that bounds the precision loss
% due to abstract interpretation of $\nn_i$.

% \begin{lemma}~\label{lem:cell}
%     For any box $B\subseteq C$, the following hold:
%     \begin{enumerate}
%         \item $\nn_k^\#(B) \subseteq [0, \delta/3]$;
%         \item if $f(B) \leq (k-1)\delta/3$, then $\nn_k^\#(B) = [0, 0]$; 
%         \item if  $f(B) \geq (k+2)\delta/3$, then  $\nn_k^\#(B) = [\delta/3, \delta/3]$
%         \aws{why k+2?}
%     \end{enumerate}
% \end{lemma}

% To prove this lemma, we will make use of the following notion:
% A \emph{minimal cover} $\cells_\boxm$ of a box $\boxm \subseteq C$ is
% the set of cells
% $\{\cell \in \cells \mid \cell \cap \boxm \neq \emptyset\}$. 
% This is a cover in the sense that $\boxm\subset \cup_{\cell \in \cells_\boxm} \cell$, and it is minimal because 
% removing any $\cell$ from $\cells_\boxm$ will make $\cells_\boxm$ not able to cover $\boxm$.

% % \begin{lemma}~\label{lem:minimal}
% %     $B\subseteq \cup_{g\in G_B}g$.
% % \end{lemma}
% % \begin{proof}
% %     Because $C\subset \cup_{g\in G}g$, then $\forall x\in B$, $\exists g'\in G$ such that $x\in g'$, and thus $B\cap g'\neq \emptyset$, so 
% %     $g' \in G_B$. 
% % \end{proof}


% \begin{proof}
%      By  the definition of $\nn_k$, $\forall x\in C$, $\nn_k(x) \in [0, \delta/3]$. Therefore, $\nn_k^\#(B) \subseteq [0, \delta/3]$. 
     
%      Because of the construction of $G$, the maximum variation 
%      of $f$ within each cell is at most $\delta/3$ (our choice of $\epsilon$ in the uniform continuity definition). 
%      \begin{enumerate}
%              \item If $f(B) \geq (k+2)\delta/3$, because $G_B$ is a minimal cover, $\forall g\in G_B$, $g\cap B\neq \emptyset$. Therefore, $\forall g\in G_B$,
%              $\exists x\in g\cap B$ such that $f(x)\geq (k+2)\delta/3$. Because the variation of $f$ in $g$ is at most $\delta/3$, then $f(g)\geq (k+2-1)\delta/3 = (k+1)\delta/3$.
%              By the definition of $U_k$, we know that $G_B\subseteq U_k$. By lemma~\ref{lem:minimal}, $B\subseteq \cup_{g\in G_B}g\subseteq \cup_{g\in U_k}g= S_k$, 
%              hence $\nn_k(x) = \delta/3$ when $x\in B$ from the construction of $\nn_k$, then $\nn_k^\#(B) = [\delta/3, \delta/3]$.
             
%              \item  Similar to the above case, if $f(B) \leq (k-1)\delta/3$, then $\forall g\in G_B$, $f(g) \leq (k-1+1)\delta/3 = k\delta/3$, hence $g\in L_k$, so if
%              $x\in B$, $\nn_k(x) = 0$, and therefore $\nn_k^\#(B) = [0, 0]$.
%      \end{enumerate}
%      This shows that $\nn_k^\#(B) = [0, 0]$ if $f(B) \leq (k-1)\delta/3$; $\nn_k^\#(B) = [\delta/3, \delta/3]$ if 
%      $f(B) \geq (k+2)\delta/3$.
% \end{proof}


% \subsection{Step 3: Putting it all together}

% \aws{N = sum of Ni}
% Let $N = \sum_{i = 0} ^ M n_i$. $N$ is the network that approximates $f$. We will prove the error introduced by $N$ is within the bound $\delta$.

% \aws{Proof of the main theorem}
% \begin{theorem}~\label{thm:simple}
%     Theorem~\ref{thm:main} holds for the simplified activation function.
% \end{theorem}
% \begin{proof}
%     Let $l = \min f(B)$ and $u = \max f(B)$. There exist some $0\leq p\leq q \leq M\in \mathbb{N}$ such that $l\in [p\delta/3, (p+1)\delta/3)$ and $u\in [q\delta/3, (q+1)\delta/3)$.
%     Moreover, let $c, d\in B$ be such that $f(c) = l$ and $f(d) = u$. 
    
%     \[N = \sum_{i = 0} ^ M n_i = \sum_{i = 0}^{p-2} n_i + \mathhl{yellow}{\sum_{i = p-1}^{p+1} n_i} + \sum_{i = p+2}^{q-2} n_i + \mathhl{yellow}{n_{q-1}}+ \sum_{i = q}^{M} n_i\]
%     We will show that the abstract interpretation of the first, the third, and the fifth terms is precise. Only the second and the forth terms (which are highlighted) could
%     possibly lose precision. If $q-p\leq 3$, the terms that lose precision are less and the bound would be tighter, so we consider the more general case.
%     \begin{mycases}
%             \case $\forall i \leq p-2$, $f(B) \geq l \geq p\delta/3\geq (i+2)\delta/3 $, then by lemma~\ref{lem:cell}, $\sum_{i = 0}^{p-2} n_i^\#(B) = \sum_{i = 0}^{p-2} [\delta/3, \delta/3]
%             = (p-1)[\delta/3, \delta/3]$ .
             
%             \case $\forall i \geq q$, $f(B) \leq u < (q+1)\delta/3 \leq (i+1)\delta/3 $, then by lemma~\ref{lem:cell}, $\sum_{i = q}^{M} n_i^\#(B) = \sum_{i = q}^{M}[0, 0] = [0, 0]$.
             
%             \case $\forall p+2\leq i\leq q-2$, 
%             \subcase $f(c) = l < (p+1)\delta/3 \leq (i-1)\delta/3$, by lemma~\ref{lem:cell}, $n_i^\#(\{c\}) = [0, 0]$;
%             \subcase $f(d)\geq q\delta/3\geq (i+2)\delta/3$, and $n_i^\#(\{d\}) = [\delta/3, \delta/3]$.
            
%             Because $\{c\}, \{d\} \subset B$, $[0, \delta/3] \subseteq n_i^\#(B)$; also by lemma~\ref{lem:cell}, $n_i^\#(B)\subseteq [0, \delta/3]$, 
%             so $n_i^\#(B) = [0, \delta/3]$ and $\sum_{i = p+2}^{q-2} n_i(B) = \sum_{i = p+2}^{q-2} [0, \delta/3]= (q-p-3)[0, \delta/3]$.

%             \case $\forall p-1\leq i\leq p+1$, because $f(d) = u \geq q\delta/3 \geq (i+2)\delta/3$,  then $n_i^\#(\{d\}) = [\delta/3, \delta/3]$, and so  $[\delta/3, \delta/3]\subseteq n_i^\#(B)$
%             by lemma~\ref{lem:cell}; $n_i^\#(B)\subseteq [0, \delta/3]$, hence $[\delta/3, \delta/3]\subseteq n_i^\#(B) \subseteq [0, \delta/3]$ and
%             $\sum_{i = p-1}^{p+1} [\delta/3, \delta/3]\subseteq  \sum_{i = p-1}^{p+1} n_i^\#(B) \subseteq  \sum_{i = p-1}^{p+1} [0, \delta/3]$. 
%             $[\delta, \delta]\subseteq \sum_{i = p-1}^{p+1}n_i^\#(B) \subseteq [0, \delta]$.
            
%             \case $i = q-1$, because $f(c) = l\leq (p+1)\delta/3\leq (i-1)\delta/3$,  then $n_i^\#(\{c\}) = [\delta/3, \delta/3]$, and so  $[\delta/3, \delta/3]\subseteq n_i^\#(B)$
%             by lemma~\ref{lem:cell}; $n_i^\#(B)\subseteq [0, \delta/3]$, hence $[0, 0]\subseteq n_i^\#(B) \subseteq [0, \delta/3]$.
    
%     \end{mycases}
    
    
    
    
%     Sum the first three cases, $(\sum_{i = 0}^{p-2} n_i + \sum_{i = p+2}^{q-2} n_i + \sum_{i = q}^{M} n_i)^\#(B) = (p-1)[\delta/3, \delta/3] +  [0, (q-p-3)\delta/3]
%     = [(p-1)\delta/3, (q-4)\delta/3]$.
    
%     Sum the remaining two cases, $[\delta, \delta]\subseteq (\sum_{i = p-1}^{p+1} n_i+n_{q-1})^\#(B)\subseteq [0, 4\delta/3]$.
    
%     Sum all terms, let $L_1 = (p+2)\delta/3$, $U_1=(q-1)\delta/3$, $L_2=(p-1)\delta/3$, $U_2=q\delta/3$, and $[L_1, U_1]\subseteq N^\#(B)\subseteq [L_2, U_2]$.
    
%     Since $l\in [p\delta/3, (p+1)\delta/3)$, then $l - \delta <(p-2)\delta/3 \leq L_2 < L_1 \leq (p+3)\delta/3\leq l+\delta$;
%     and $u\in [q\delta/3, (q+1)\delta/3)$, then $u - \delta < (q-2)\delta/3 \leq U_1 < U_2 \leq (q+3)\delta/3\leq u+\delta$. 
%     Therefore, $[l+\delta, u-\delta] \subseteq N^\#(B) \subseteq [l-\delta, u+\delta]$.
    
% \end{proof}



% \begin{figure}[t!]
%     \footnotesize
%     \begin{center}
%         \begin{tikzpicture}

%             % \draw node at (6, 3 ) [input] (in) {$\bx$};


%             % nodes
%             \draw node at (0.2, 1) [empty] (nn0) {$\nn_0$};
%             \draw node at (1, 1) [oper] (op1) {$\act_{\cell_1}$};
%             \draw node at (2, 1) [oper] (op2) {$\act_{\cell_2}$};
%             \draw node at (3, 1) [empty] (op3) {$\cdots$};
%             \draw node at (4, 1) [oper] (op4) {$\act_{\cell_{|U_0|}}$};
%             \draw[dashed] (0.5,0.5) rectangle (4.6,1.5);

%             \draw node at (6, 1) [empty] (op5) {$\cdots$};

%             \draw node at (7.2, 1) [empty] (nnm) {$\nn_M$};
%             \draw node at (8, 1) [oper] (op6) {$\act_{\cell_1}$};
%             \draw node at (9, 1) [empty] (op7) {$\cdots$};
%             \draw node at (10, 1) [oper] (op8) {$\act_{\cell_{|U_M|}}$};
%             \draw[dashed] (7.5,0.5) rectangle (10.6,1.5);

%             \draw node at (2.5,-1) [oper] (s) {$\sum$};
%             % \draw node at (4, 0) [output] (out) {$y$};

%             \draw[->,thick] (op1) -- (s);
%             \draw[->,thick] (op2) -- (s);
%             \draw[->,thick,dashed] (op3) -- (s);
%             \draw[->,thick] (op4) -- (s);

%             \draw node at (9,-1) [oper] (s2) {$\sum$};

%             \draw[->,thick] (op6) -- (s2);
%             \draw[->,thick,dashed] (op7) -- (s2);
%             \draw[->,thick] (op8) -- (s2);

%             \draw node at (6,-1) [empty] (d) {$\cdots$};
%             \draw node at (6,-2) [oper] (s3) {$\sum$};
%             \draw[->,thick] (s) -- (s3);
%             \draw[->,thick] (s2) -- (s3);
%             % \draw[->,thick,dashed] (d) -- (s3);

%             \draw[->,thick] (s3) -- (6,-3);

%             % \draw node at (4, 0) [output] (out) {$y$};

%             % \draw[->,thick] (op) -- (out);

      
%         \end{tikzpicture}
%         \caption{The neural network $\nn$ constructed for the simplified case (\cref{sec:linear}).
%         Each of the step activation functions receives as input the entire input vector $\bx$ (not shown).}
%         \label{fig:simple}
%     \end{center}
% \end{figure}

==> general.tex <==
\section{Generalized Abstract Universal Approximation}
\label{sec:general}

==> outline.tex <==

\section{Proof Outline of the AUA Theorem}\label{sec:outline}

In this section, we give an outline of the proof of the AUA theorem.

%
Our proof proceeds by constructing a neural network $\nn$
and showing that it $\delta$-abstractly approximates a continuous  function $f$.  
%
The precision loss $\delta$ 
comes from two sources, approximation and abstract interpretation.
Our proof carefully constructs a neural network that controls both sources of imprecision.
%
The construction of $\nn$ is divided into four steps,
described in \cref{sec:step1,sec:step2,sec:step3,sec:step4}, respectively.
Our high-level proof outline resembles that of \citet{univ_cert}
for ReLU networks.
However, our construction of the neural network and analysis 
are necessarily different, and more challenging,
 due to our need to work with arbitrary activation functions.

\begin{table}
    \footnotesize
    \begin{tabular}{lp{9cm}l}
        \toprule
        Symbol & Meaning & Definition location\\
        \midrule
        $f$ & The continuous function $f: C \to \R$ that we wish to approximate & \cref{thm:main} \\
        $\delta$ &  Allowed approximation error from theorem statement & \cref{thm:main}\\
        $\act$ & A fixed limit-bounded function used to construct the approximation $\nn$ & \cref{thm:main}\\
        ~\\
        $f_i$ & The $i$th slice of function $f$ & Step 1; \cref{sec:step1}\\
        $\unit$ & Slice size $\unit = \delta/3$ & Step 1; \cref{sec:step1}\\
        $K$ & The number of slices of $f$ is $K+1$ & Step 1; \cref{sec:step1}\\
        ~\\
        $\epsilon$ & Size of the grid cell & Step 2; \cref{sec:step2grid}\\
        $\cells$ & Set of all boxes in the $\epsilon$-grid & Step 2; \cref{sec:step2grid}\\
        $\cell$ & A box in  the $\epsilon$-grid & Step 2; \cref{sec:step2grid}\\ 
        $\lprec$ & The loss of precision due to the limit behavior of $\act$& Step 2; \cref{sec:step21d}\\
        $\dilate$ & Dilation factor used to approximate sign functions with activations & Step 2; \cref{sec:step21d}\\
        $\bumpi$ & Simple neural network approximating a step function & Step 2; \cref{sec:step21d}\\
        $\bumpc$ & Neural network that indicates whether an input is in box $\cell$ of $\epsilon$-grid
         & Step 2; \cref{sec:step2md}\\
        ~\\
        $\nn_i$ & Neural network approximating the $i$th function slice $f_i$ & Step 3; \cref{sec:step3}\\
        $\nn$ & The neural network approximating $f$ & Step 4; \cref{sec:step4}\\
        \bottomrule
    \end{tabular}
    \caption{Symbols used in the proof of the AUA theorem, organized by proof step}
    \label{tbl:symbols}
\end{table}

    \paragraph{Step 1: Function slicing}
    We begin our construction by \emph{slicing} the function $f$ 
    into a sequence of functions $f_i$, such that $f = \sum_i f_i$.
    Each  $f_i$ captures
    the behavior of $f$ on a small interval of its range.
    In the next steps, we approximate each function slice $f_i$
    using a neural network $\nn_i$.
    By slicing the range of function $f$, 
    we control precision loss due to approximation.

    
    \paragraph{Step 2: $\epsilon$-grids and indicator functions}
    This step is the most challenging part of the construction.
    Our approximation $\nn_i$ of function slice $f_i$
    need only  capture extremal values: $f_i(\bx)$ is \emph{high}
    or \emph{low}. 
    Since the range of $f_i$ is small, precision loss is bounded,
    despite this rough approximation.
%
%
    In this step, 
    we divide the input domain $C$ into a grid of boxes,
    and construct a series of neural networks that indicate whether
    an input $\bx$ is in a specific box in the grid---\emph{high} or \emph{low}.
    %
    These neural networks approximate \emph{indicator} functions:
    roughly 1 within the desired region, and roughly 0 elsewhere.
    The challenge is to (1) approximate indicator functions using 
    arbitrary activation functions and (2) prove that the loss of precision 
     is bounded. 


    \paragraph{Step 3: Slice approximation}
    At this point in the proof, we 
    use our  indicator-function approximations from Step 2 to 
    construct a  neural network $\nn_i$ approximating
    each function slice $f_i$.
    Essentially, $\nn_i$ uses indicator functions to
    check whether an input is in a \emph{high} or \emph{low}
    region of the grid, and outputs the appropriate value accordingly.

    \paragraph{Step 4: Composing slice approximations}
    Finally, we compose all $\nn_i$ into a single neural network $\nn$
    that approximates the function $f$.
    Following the properties of $\nn_i$, we show that $\nn$ satisfies
    AUA theorem. 


% The proof of the general AUA theorem follows the above structure.
% The key difference from our simplified setting in this section
% will be in Step 2. Since we are given arbitrary limit-bounded activation functions in the general setting,
% we need to carefully work with them to get a good approximation of slices
% and limit precision loss of abstract transformers.


%

In what follows, we will formalize and illustrate all steps of the proof.
\cref{tbl:symbols} lists all of the primary symbols used in the theorem
statement and throughout the proof. Throughout the paper, when we say \emph{imprecision}, 
we mean the discrepancy between the abstract interpretation of the neural network 
and the set semantics of the approximated function. 

==> slice.tex <==
\input{ill_step3}

\section{Proof Step 3: Slice Approximation}\label{sec:step3}
Having constructed the indicator function $\nn_\cell$ for each box $\cell\in \cells$, we  are now ready to build the neural network $\nn_i$ that approximates the function slice $f_i : C \to [0,\unit]$. 

Recall that, in Step 1 (\cref{sec:step1}),
we sliced the range of  $f$ into 
$\left[0, \unit\right],\left[\unit, 2\unit\right], \ldots, \left[K\unit, u\right]$,
and defined a 
sequence of $K+1$ function slices of the form:
%
\[ 
  f_i(\bx)=\begin{cases}
               f(\bx) - i \unit, & i \unit < f(\bx) \leq (i + 1)\unit \\
               0, & f(\bx) \leq i\unit \\
               \unit, &(i+1) \unit < f(\bx)
            \end{cases}
\]
Our approximation of $f_i$ will be coarse:
all we need to capture is whether the value of $f_i$
is $\unit$; otherwise, we will consider the value to be $0$.

%
If we amplify $f_i$ by $\frac{1}{\unit}$, i.e., consider $\frac{1}{\unit}f_i(\bx)$, it is roughly similar to an indicator function for the set $S = \{\bx \in C \mid f(\bx)> (i+1)\unit\}$, i.e., 
indicating when $f(\bx)$ is greater than the upper bound of the $i$th slice.
To approximate this behavior, 
we will consider all boxes in $\cells$ that are subsets of $S$,
and construct an  indicator function to tell us whether an input
$\bx$ is in those boxes, as follows:

Let $\cells_i \subseteq \cells$ 
be the set of boxes 
in which the value of $f(\bx)$ is greater than the upper bound of the $i$th slice, $[i\unit, (i+1)\unit]$:
\[
    \cells_i = \{\cell\in \cells\mid f(\cell)> (i+1)\unit\} 
\] 
%

\begin{figure}

    \begin{subfigure}{.3\textwidth}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                axis lines=middle,
                xmax=5.2,
                xmin=0,
                ymin=0,
                ymax=0.55,
                ytick={0,.4},
                xtick={0,1,2,3,4,5},
                height=0.4cm,
                width=3cm
            ]
          
            \addplot [domain=-1:5, samples=100, thick, blue] {max(min(sin(deg(2*x))+1, 1.6), 1.2)-1.2};
            %\addplot [mark=none,thick, dotted]  {\foreach \x in {0.2, 0.4, ..., 5.0} coordinates (\x, 0) (\x, 2)};
            \pgfplotsinvokeforeach{0.5,1.0,...,5}{\addplot[mark=none,gray] coordinates { (#1,0) (#1,.4) };}
            \draw[thick, white, fill=red,opacity=0.15] (0.5,0) rectangle (1,.4);
            \draw[thick, white, fill=red,opacity=0.15] (3.5,0) rectangle (4,.4);
          \end{axis}
          %\draw [dashed] (0,1) -- (1,1);
        \end{tikzpicture}
        \caption{$f_3$ with $0.5$-grid}\label{fig:grid_f3}


    \end{subfigure}
%
%
    \begin{subfigure}{.68\textwidth}
        \footnotesize
        \begin{center}
            \begin{tikzpicture}
                % nodes
                \draw node at (-.5, 0) [input] (in) {$x_1$};
                \draw node at (-.5, -2) [input] (in2) {$x_m$};
                \draw node at (-.5, -.9) [input] (dots) {$\vdots$};
        
                \draw node at (1, 0) [oper] (plus) {$\nn_{\cell_1}$};
                \draw node at (1, -.9) [input] (dots2) {$\vdots$};
        
        
        
                \draw node at (1, -2) [oper] (plus1) {$\nn_{\cell_{|\cells_i|}}$};
                
        
                \draw node at (2, -1) [oper] (sum) {$\sum$};
                \draw node at (3.5, -1) [oper] (act) {$\act$};
        
                \draw[->,thick] (in) -- (plus);
                \draw[->,thick] (in2) -- (plus1);
                \draw[->,thick] (in) -- (plus1);
                \draw[->,thick] (in2) -- (plus);

                \draw[->,dotted] (in) -- (dots2);
                \draw[->,dotted] (in2) -- (dots2);

                \draw[->,thick] (plus) -- (sum);
                \draw[->,thick] (plus1) -- (sum);
                \draw[->,thick] (sum) to node[above]{$\dilate$} (act);
                \draw[->,thick] (act) -- (4.5,-1);            
            \end{tikzpicture}
        \end{center}
        \caption{Illustration of $\nn_i$ (added constants elided), where $\bumpc$ is used as a black 
        box.
        Note how each $\bumpc$ receives all $m$ inputs of the neural network.}
        \label{fig:nni}
        \end{subfigure}
        \caption{\textbf{Step 3} Illustration}
    \end{figure}

\begin{example}
    Consider \cref{fig:grid_f3},
    which shows function slice $f_3$ from our running example.
   %
    We have constructed a $0.5$-grid over the 1-dimensional input domain.
    The two highlighted boxes comprise the set $\cells_3$---every box where the
    value of $f_3$ is $\unit = 0.4$.
    Note that, in general, the set $\cells_i$ may contain overlapping boxes,
    but in this example we do not observe such case.
\end{example}



Define $\nn_i$ that approximates $\frac{1}{\unit}f_i(\bx)$ as
\[\nn_i(\bx) = \act \left( \dilate \left( \sum_{\cell\in\cells_i}\bumpc(\bx)-0.5 \right) \right)\]
\cref{fig:nni} shows $\nn_i$ as a graph.
Informally, $\nn_i$ encodes the following:
If $\bx$ is in a box where $f_i$ is greater than the upper bound of the $i$th slice ($\bumpc(\bx) \approx 1$), 
then return $\approx1$; otherwise, return $\approx 0$.
The outer activation function, as with the construction of $\bumpc$, acts as a sign  function.

%\zw{\emph{Why considering all boxes in $\cells$} It may appear unnecessary to consider all boxes $\cell\in\cells$ such that $f(\cell)\geq (i+1)\unit$. Instead we could 
%only consider the maximum one. However, we need to accommodate the abstract semantics, i.e., for any box $B$ in $C$, we need that $\nna_i$ has the similar property as in 
%the indicator function. Because our construction considers all boxes in $\cells$, then $B$ will have an approximation $\cell$ in the grid, and }

% Before proving the properties of $\nna_i$, we first discuss the neighborhood hyperrectangle in the gird of a box $\boxm$, which helps us establish the 
% properties.

% \paragraph{Neighborhood hyperrectangle in the gird containing a box $\boxm$}
% In~\cref{sec:step2}, we have defined the immediate neighbors for $\cell\in \cells$. Now we extend this definition to all boxes in $C$. For a box $\boxm \subset C$,
% if $\boxm\in \cells$, then $\boxm$'s neighborhood $\cell_\boxm = \ngbr(\boxm)$; otherwise, let $\cell_\boxm$ be the minimum $\cell \in \cells$ such that $\boxm\subseteq \cell$. It is minimum 
% in the sense that if $\exists \cell'\in \cells$ such that $\boxm\subseteq \cell'$, then $\cell_\boxm\subseteq \cell'$.

% \begin{lemma}[Coordinate Representation of Neighborhood Hyperrectangle]\label{lem:cord}
%     Let $\cell_\boxm$ have the representation $[a_1, b_1]\times\ldots\times[a_m, b_m]$ and $\boxm$ have the representation $[a'_1, b'_1]\times\ldots\times[a'_m, b'_m]$, then 
%     $\forall i\in\{1,\ldots, m\}$, $-\epsilon \leq a_i - a'_i \leq 0$ and $0 \leq b_i - b'_i \leq \epsilon$.
% \end{lemma}

% \begin{proof}
%     Because $\boxm\subseteq \cell_\boxm$, $\forall i\in\{1,\ldots, m\}$, $a_i - a'_i \leq 0$ and $b_i - b'_i\geq 0$; and $\cell_\boxm$ is minimum, so 
%     $\forall i\in\{1,\ldots, m\}$, $a_i - a'_i \geq -\epsilon$ and $b_i - b'_i \leq \epsilon$; otherwise, we can either add $\epsilon$ to 
%     $a_i$ or substract $\epsilon$ from $b_i$ to get a smaller $\cell'$ such that $\boxm\subseteq \cell'$.
    
%     Thus, $\forall i\in\{1,\ldots, m\}$, $-\epsilon \leq a_i - a'_i \leq 0$ and $0 \leq b_i - b'_i \leq \epsilon$.
% \end{proof}

% \begin{lemma}\label{lem:min_rect}
%     $\forall \bx\in \cell_\boxm$, $\exists \by\in \boxm$, such that $||\bx-\by||_\infty \leq \epsilon$.
% \end{lemma}
% \begin{proof}
%     From~\cref{lem:cord}, let $\boxm$ have the representation $[a'_1, b'_1]\times\ldots\times[a'_m, b'_m]$ and $\cell_\boxm$ have the representation 
%     $[a_1, b_1]\times\ldots\times[a_m, b_m]$, then $\forall i\in\{1,\ldots, m\}$, $-\epsilon \leq a_i - a'_i \leq 0$ and $0 \leq b_i - b'_i \leq \epsilon$.
    
%     $\forall \bx\in \cell_\boxm$, we will construct such a $\by\in \boxm$:

%     If $\bx\in \boxm$, let $\by = \bx$;

%     If $\bx\in \cell_\boxm\setminus \boxm$.
%     For each $i\in \{1,\ldots,m\}$, 
%     \begin{enumerate}
%         \item If $x_i\in [a'_i, b_i']$, then let $y_i = x_i$. 
%         \item if $x_i<a'_i$, then let $y_i = a'_i$. 
        
%         Because $\bx\in \cell_\boxm$, $x_i\geq a_i$, and we have $a_i - a'_i \geq -\epsilon$, then 
%         $x_i\geq a_i\geq a'_i -\epsilon$. From $x_i<a'_i$ and $x_i\geq a'_i-\epsilon$, so $|a'_i - x_i|\leq\epsilon$.

%         \item If $x_i>b'_i$, let $y_i = b'_i$. 
        
%         Because $\bx\in \cell_\boxm$, $x_i\leq b_i$, and we have $b_i - b'_i \leq \epsilon$, then 
%         $x_i\leq b_i\leq b_i' +\epsilon$. From $x_i > b'_i$ and $x_i\leq b'_i+\epsilon$, so $|b'_i - x_i|\leq\epsilon$.
%     \end{enumerate}
%     We have constructed a $\by\in \boxm$, and $||\bx-\by||_\infty \leq \epsilon$.
% \end{proof}

% \aws{still not clear}
% \paragraph{Abstract precision of $\nn_i$}
% \zw{Because we consider all $\cell\in\cells$ such that $f(\cell)\geq (i+1)\unit$, the abstract semantics is also encoded in $\nn_i$. 
% For any box $\boxm$ in $C$,  we need that $\nna_i$ has the similar property as in the indicator function that if $B\subset S$ then $\nna_i(B) = 1$. Because boxes in the grid 
% form an approximation for boxes in $C$, $\boxm$'s counterpart in the grid satisfies the indicator property, and thus $\boxm$ also satisfies it.}
% \aws{the above sentences are not very clear. (1) what "properties" are you referring to? (2) Is this the right place for this description or in the next part on abstract precision. } 
% We now discuss properties of the abstract interpretation of $\nn_i$.
% We begin by proving a lemma about the behavior
% of $f$ on a box $\boxm$.

% \aws{say why we need neighborhood of B?}


\paragraph{Abstract precision of $\nn_i$}
Observe how for any box $\boxm \subseteq C$ from the abstract domain, it is overapproximated by a larger box $\cell \supseteq \boxm$ from the finitely many boxes in the $\epsilon$-grid.
Intuitively,
our abstract approximation of $\nn_i$ incurs an 
error when the input $\boxm$ is not in the grid.
We formalize this idea by extending the notion of neighborhood (\cref{sec:step2grid}) 
to boxes from the abstract domain.

% In \, we defined the neighborhood for a box $\cell\in \cells$.
% Now we extend this definition to all boxes in $C$. 
For a box $\boxm \subseteq C$, 
if $\boxm\in \cells$, then $\boxm$'s neighborhood $\cell_\boxm = \ngbr(\boxm)$; otherwise, let $\cell_\boxm$ be the smallest $\cell \in \cells$, by volume, such that $\boxm\subseteq \cell$.
Note that $\cell_\boxm$ is uniquely defined. 
% It is minimum 
% in the sense that if $\exists \cell'\in \cells$ such that $\boxm\subseteq \cell'$, then $\cell_\boxm\subseteq \cell'$.
%
The following lemma says that considering the neighborhood of $\boxm$ only adds up to $\unit$
of imprecision to the collecting semantics of $f$.

%\todo{what happens if $B = C$}

\begin{lemma}[Properties of $\cell_\boxm$]
    \label{lem:var}
    The following is true:
    \begin{enumerate}
        \item If $f(\boxm) \geq \beta$, then $f(\cell_\boxm)\geq \beta-\unit$.
        \item If $f(\boxm) \leq \beta$, then $f(\cell_\boxm)\leq \beta+\unit$.
    \end{enumerate}
\end{lemma}




Finally, the following theorem 
states that the abstract interpretation, $\nn_i^\#(\boxm)$,
returns a box that is almost $1$
when $f(\boxm)$ is above the upper bound of the $(i+1)$th 
slice, and almost $0$ when $f(\boxm)$
is below the lower bound of the  $(i-1)$th slice.
This theorem is illustrated in \cref{fig:step3_thm}.
Note that the theorem does not
make any claims about the behavior
of $\nna_i(\boxm)$ 
if the $i$th slice overlaps with $f(\boxm)$
or is adjacent to those that overlap with $f(\boxm)$---these 
are the slices that are not highlighted in purple in \cref{fig:step3_thm},
i.e., slices 2--7.


\begin{theorem}[Abstract interpretation of $\bumpc$]\label{thm:abs_slice}
    For any box $\boxm \subseteq C$, let $u = \max f(\boxm)$, and $l = \min f(\boxm)$. The following is true:
    \begin{enumerate}
        \item $\nna_i(\boxm)\subseteq [0, 1]$.
        \item If $l\geq (i+2)\unit$, then\  $\exists u_i\in (1-\lprec, 1]$ such that $[u_i, u_i] \subseteq \nna_i(\boxm)\subseteq (1-\lprec, 1]$.
        \item If $u\leq  (i-1)\unit$, then\  $\exists l_i\in [0, \lprec)$ such that $[l_i, l_i] \subseteq \nna_i(\boxm)\subseteq [0, \lprec)$.
    \end{enumerate}
\end{theorem}

In Statements (2) and (3), 
the lower bounds $[u_i, u_i]$ and $[l_i, l_i]$ will be needed when we analyze  $\nna(\boxm)$ in the main theorem;
there, we  will
need to derive under- and overapproximations
of
 the box $\nna(\boxm)$.

\input{ill_step3_thm}


\begin{proof}
    We begin by noting that in Statement (2), $[u_i, u_i] \subseteq \nna_i(\boxm)$ for some $u_i\in (1-\lprec, 1]$ is a direct corollary of $\nna_i(\boxm)\subseteq (1-\lprec, 1]$. 
    Because if $\nna_i(\boxm)\subseteq (1-\lprec, 1]$, and $\nna_i(\boxm)\neq \emptyset$, then $\nna_i(\boxm)$ contains at least one point in $(1-\lprec, 1]$.
    %
    Similarly, in Statement (3), $[l_i, l_i] \subseteq \nna_i(\boxm)$ for some $l_i\in [0, \lprec)$ is a direct corollary of $\nna_i(\boxm)\subseteq [0, \lprec)$.

    Because the limit precision $\lprec$ is our choice, and we have chosen  $\lprec\leq \frac{1}{K+1}$ (see~\cref{sec:step21d}), we can also enforce  that $\lprec\leq \frac{1}{4|\cells|}$,
    a fact we will use later in the proof.

    \vspace{0.5em}\noindent
    \textsc{Statement (1):}
        The outer function of $\nn_i$ is $\act$, whose range is $[0,1]$, by the definition of limit-boundedness and our construction, so $\nna_i(\boxm)\subseteq [0, 1]$.

    \vspace{0.5em}\noindent
    \textsc{Statement (2):}
        Because $f(\boxm)\geq (i+2)\unit$, by \cref{lem:var}, $f(\cell_\boxm)\geq (i+1)\unit$, so $\cell_\boxm\in \cells_i$.
        Thus, we can break up the sum as follows:
        \[
            \sum_{\cell\in\cells_i}\bumpc(\bx)  = \left(\sum_{\cell\in(\cells_i\setminus \{\cell_\boxm\})}\bumpc(\bx)\right) + \nn_{\cell_\boxm}(\bx)  
        \]

        From~\cref{thm:abs_bump}, $\nna_{\cell_\boxm}(\boxm)\subseteq (1-\lprec, 1]$, and $\absbumpc(\boxm)\subseteq [0,1]$ for $\cell\in\cells_i\setminus \{\cell_\boxm\}$.
        Therefore, we can conclude the following two facts:
        \[\sum_{\cell\in\cells_i}\absbumpc(\boxm)\subseteq (1-\lprec, \infty)
         \quad\quad \text{and} \quad\quad
        \sum_{\cell\in\cells_i}\absbumpc(\boxm) \absplus \left[-0.5,-0.5\right]\subseteq \left(0.5-\lprec, \infty\right)
        \subset \left(0.5\epsilon, \infty\right)\] 
        %\zw{?} 
        %\aws{yes why not}
        The second inequality follows from the fact that we assumed $\lprec \leq \frac{1}{4|\cells|} \leq 0.25$ (above) and $\epsilon< 0.5$ (see~\cref{sec:step2grid}). Therefore, $0.5-\lprec > 0.25>0.5\epsilon$.
        %\aws{where did $0.5\epsilon$ come from? there's a lemma way back, mention it}
        % Hence,\[
        %     \sum_{\cell\in\cells_i}\absbumpc(\boxm) \absplus -\left(0.5\right)^\# \subset \left(0.5\epsilon, \infty\right)
        % \]

        It follows from~\cref{lem:dilate} that 
        \[
        \nna_i(\boxm) = \absact \left( \dilate^\#\abstimes\left(\sum_{\cell\in\cells_i}\absbumpc(\boxm) \absplus \left[-0.5,-0.5\right]\right)\right)\subseteq (1-\lprec, 1]
        \]

      %  \aws{same thing above, break up the simplification into more steps, and cite lemma on limits}

    \vspace{0.5em}\noindent
    \textsc{Statement (3):}
        If  $u\leq  (i-1)\unit$, we will show that $\forall \cell\in \cells_i\ldotp \boxm\subset C\setminus\ngbr(\cell)$. %\aws{not very clear why}.

        Pick any $\cell \in \cells_i$, then we have $f(\cell)\geq (i+1)\unit$. Thus, from~\cref{lem:var}, 
        $f(\cell_\boxm)\geq i\unit$. Recall that if $\boxm\in \cells$, then $\cell_\boxm = \ngbr(\boxm)$. Hence, $f(\ngbr(\cell))\geq i\unit$.
        %
        However, $f(\boxm)\leq u\leq (i-1)\unit$, so $\boxm\cap \ngbr(\cell)=\emptyset$. Equivalently, $\boxm\subset C\setminus\ngbr(\cell)$.
%
       % \aws{use more intuition above. Break sentences with periods, as its unclear what implies what.}
%

        From~\cref{thm:abs_bump}, $\forall \cell \in \cells_i\ldotp \absbumpc(\boxm)\subseteq [0, \lprec)$, so 
        \[\sum_{\cell\in\cells_i}\absbumpc(\boxm)\subseteq [0, |\cells_i|\lprec)\subseteq  [0, |\cells|\lprec)\]


        We assumed that $\lprec \leq \frac{1}{4|\cells|}$ and $\epsilon< 0.5$ (see~\cref{sec:step2grid}), so $|\cells|\lprec\leq 0.25$, 
        and $|\cells|\lprec - 0.5\leq -0.25\leq -0.5\epsilon$. Hence,
%
        \[\sum_{\cell\in\cells_i}\absbumpc(\boxm)\subseteq[0, 0.25)
        \quad\quad\text{and}\quad\quad
        \sum_{\cell\in\cells_i}\absbumpc(\boxm) \absplus \left[-0.5,-0.5\right] \subseteq \left[-0.5, -0.25\right)\subseteq \left(-\infty, -0.5\epsilon\right)\]
        
        It follows from~\cref{lem:dilate} that
        \[\nna_i(\boxm) = \absact \left( \dilate^\#\abstimes\left(\sum_{\cell\in\cells_i}\absbumpc(\boxm) \absplus \left[-0.5,-0.5\right]\right)\right) \subseteq [0, \lprec)\]

      %  \aws{break the above into different lines. $|\cells|$ should be $|\cells_i|$. Add more english and references, why 0.25...because $V=...$}

\end{proof}




\section{Proof Step 4: Sum all approximating slices}\label{sec:step4}
We have arrived at the final step of the proof,
where we construct a neural network $\nn$ to $\delta$-abstractly approximate $f$.

Because each $\nn_i$ from Step 3 is an approximation for $\frac{1}{\unit}f_i$ and $\sum_{i=0}^K f_i = f$, we will construct the neural network $\nn$ as 
\[\nn(\bx) = \unit\sum_{i=0}^K \nn_i (\bx)\]
%
We will show that $\nn$ $\delta$-abstractly approximates $f$, which will conclude~\cref{thm:main}. Formally:
For every box $\boxm\subseteq C$, \[[l+\delta, u-\delta] \subseteq \ \nna(\boxm) \  \subseteq [l-\delta, u+\delta]\] 
where $l = \min f(\boxm)$ and $u = \max f(\boxm)$.



Before proceeding with the proof,
we give a general lemma 
that will be useful in our analysis.
The lemma follows from the fact that, by construction,
$\lprec \leq \frac{1}{K+1}$.

\begin{lemma}\label{lem:ineq}
    If $\eta_0,\ldots,\eta_K \in [-\lprec, \lprec]$, then $\sum_{i=0}^K \eta_i \in[-1, 1]$.
\end{lemma}

% We need this inequality to show that the imprecision introduced by the limit of the activation function 
% is bounded by $0.5\unit$ propagated from all the $K+1$ slices $\nn_i$ (see~\cref{sec:step21d}).
% We can substitute $(\pm)l_i$, $(\pm)\lprec$ and $(\pm)(1-u_i)$ to $\eta_i$ in~\cref{lem:ineq}. 
% Recall that $u_i\in(1-\lprec, 1]$ and $l_i\in[0,\lprec)$ in~\cref{thm:abs_slice}, so $1-u_i\in[0, \lprec)$.
% \aws{what are $u_i$ and $l_i$}
% \aws{the above paragraph doesn't make sense}
% \zw{I also added a remark at the end of~\cref{thm:abs_slice} to explain $l_i$ and $u_i$}


    \paragraph{Proof outline} Our proof of \cref{thm:main} involves three pieces,
    outlined below:
    \begin{enumerate}[label=(\Alph*)]
        \item Because $\nna(\boxm) = \unit^\#\abstimes \sum_{i=0}^K \nn_i^\#(B)$, we need only analyze $\sum_{i=0}^K \nn_i^\#(B)$.
         We will decompose the sum into five sums and analyze each separately,
         arriving at five results of the form: 
         $$\left[\tilde{L}_{1j}, \tilde{U}_{1j}\right]\subseteq \sum_{i\in S_j} \nn_i^\#(B)\subseteq \left[\tilde{L}_{2j}, \tilde{U}_{2j}\right]$$ 
         for $j\in\{1,\ldots,5\}$, where $\bigcup_j S_j = \{0,\ldots,K\}$
         and $S_j$ are mutually disjoint sets.
        
         \item Then, we sum over all five cases, getting 
        $$\left[\sum_{j=1}^5\tilde{L}_{1j}, \sum_{j=1}^5\tilde{U}_{1j}\right]\subseteq \sum_{i=0}^K \nn_i^\#(B)\subseteq \left[\sum_{j=1}^5\tilde{L}_{2j}, \sum_{j=1}^5\tilde{U}_{2j}\right]$$

        \item Let $L_i = \unit\sum_{j=1}^5\tilde{L}_{ij}$ and $U_i = \unit\sum_{j=1}^5\tilde{U}_{ij}$. Then, we get the bound $[L_1, U_1]\subseteq \nna(\boxm) \subseteq [L_2, U_2]$.
        
        Finally, we show that 
        $[L_2, U_2]\subseteq [l-\delta, u+\delta]$ and $[l+\delta, u-\delta]\subseteq [L_1, U_1]$.

        Equivalently, we will show that
        \[l-\delta \leq L_2\leq L_1 \leq l+\delta  \quad \text{ and } \quad u-\delta \leq U_1 \leq U_2 \leq u+\delta\]
    \end{enumerate}
    
   
    %


\paragraph{Proof assumptions}
    We will assume that $l\in [p\unit, (p+1)\unit)$ and $u\in [q\unit, (q+1)\unit)$, for some $p\leq q\leq K$.
    Additionally,  
    let $c, d\in B$ be such that $f(c) = l$ and $f(d) = u$.


  \paragraph{Step A: Decompose sum and analyze separately}  
  We begin by decomposing the sum into five terms. 
%
  We start with an informal explanation of why we decompose the sum this way,
  and illustrate the process in   \cref{fig:nn_approx}.
%
  %\todo{These next 3 paragraphs are supposed to be intuition for how we break up the terms. Just refer to the figure and \cref{thm:abs_slice} for the intuition.
%Currently, it's hard-to-follow inequalities. Feel free to add more things to the figure; e.g., Term 1 precise, Term 2; not precise, etc.}

  This is the most important step of the proof. We want to show that most $\nn_i$'s in $\sum_{i=0}^K \nn_i^\#(\boxm)$ are (almost) precise. 
  %
  %\todo{just say by almost, we mean they return $\approx 1$ where they're supposed to.
  %I don't think this is the place to talk about limits.
  %We've known all along that limits are precision-loss factors.}
%
  By almost we mean that their values are $\approx 1$ and $\approx 0$.
  %we mean that because 
  %we can only control the activation function $\act$ at its limit is within a tiny range as in~\cref{sec:step21d}. \aws{mention specific theorem; mention $\lprec$ that's all u r referring to} But if $\act$ could achieve its limits at both sides, i.e.,  $\exists D>0$ such that $\forall x>D\ldotp\act(x) = \lim_{x\rightarrow\infty}\act(x)$
  %and $\forall x<-D\ldotp\act(x) = \lim_{x\rightarrow-\infty}\act(x)$, then $\lprec = 0$ and most of the terms would be precise.
  %\aws{what does precise mean here. the sentence about limit needs rewriting}\zw{I think we should mention somewhere, when we say precise, we mean their set semantics and the interval semantics are the same.}
  %
  The motivation is then to extract as many precise terms as possible. The only tool used in the analysis is~\cref{thm:abs_slice}. %If we can show that $f(\boxm)\geq (i+2)\unit$ or $f(\boxm)\leq (i-1)\unit$, we know that 
  %the abstract interpretation of those $\nn_i$'s are (almost) $1$ or $0$,
  %a fact that follows from \cref{thm:abs_slice}. 
  %

  \begin{itemize}
    \item 
    %As shown in~\cref{fig:nn_approx}, $f(\boxm) = [l, u]$. %$i\leq p-2$, $(i+2)\unit\leq p\unit\leq l = \min f(B)$. 
    Consider the function slices represented by Term 1 and 5;
    for example, Term 1 represents abstractions $\nna_i$
    of function slices $f_i$, for $i \in [0,p-2]$. 
    The function slices of Term 1 and 5 are referred to in 
    \cref{thm:abs_slice} (Statements 2 and 3):
    they have an (almost) precise abstract interpretation.
    That is, the abstract semantics of $\nna_i(\boxm)$ and the collecting semantics of $f_i(\boxm)$ agree.
  For Term 1,
  the abstract interpretation of all $\nna_i(\boxm) \approx [1,1]$
  and $f_i(\boxm) = [\unit,\unit]$.
  For Term 5, 
  the abstract interpretation of all $\nna_i(\boxm) \approx [0,0]$
  and $f_i(\boxm) = [0,0]$.
  %\aws{$f(B) = u$ and $l$ don't typecheck}
  %  \aws{what is meant by slice here? function slices?}

  \item 
%   For function slices $f_i$ where $i \in [p-1, q+1]$, if there are many of them, i.e., $q\gg p$, we can also show that most of them are (almost) precise. 
%    The abstract semantics of 
%   $\nna_i(\boxm)\approx [0,1]$\zw{Is this an abuse of $\approx$?} and the set semantics of $\frac{1}{\unit}f_i(\boxm)=[0, 1]$.
  Now consider function slices $f_i$, where $i \in [p+2,q-2]$; see Term 3 in \cref{fig:nn_approx}.
  The abstraction of these function slices is also (almost) precise.
  We can see $f(c) = l$ is below the lower bound of 
  the slices and $f(d) = u$ is above the upper bound of the slices. Hence, $f_i(d) = \unit$ and 
  $\nna_i(\alpha(\{d\})) \approx [1,1]$.
  Similarly, $f_i(c) = 0$ and
  $\nna_i(\alpha(\{c\})) \approx [0,0]$. Because $c, d\in \boxm$, and due to continuity of $f$, we have  $f_i(\boxm) = [0, 1]$, 
  and  $\nna_i(\boxm)\approx[0, 1]$.
  
  \item 
  The remaining function slices are those in Term 2 and Term 4, and they are at the neighborhood of the boundary of $[l, u]$. Most precision loss  
 of $\nna_i(\boxm)$ comes from those two terms.

  \end{itemize}
  %$\forall i\in\{0,\ldots, K\}$, we know that $\nna_i(\boxm)\subseteq[0, 1]$. 
  %\aws{what is $i$ here? how do we know that$f(c) = l\leq (i-1)\unit$ }
  %For $p+2 \leq i\leq q-2$, we have $f(c) = l < (p+1)\unit\leq (i-1)\unit$;
  %so $\nna_i(\alpha(\{c\}))$ is close to $0$. Similarly, $f(d) = u\geq q\unit\geq (i+2)\unit$, so $\nna_i(\alpha(\{d\}))$ is close to $1$. Because, $\{c\}, \{d\}\subseteq \boxm$, then $[\approx 0, \approx 1]\subseteq\nna_i(\boxm)\subseteq[0, 1]$.
  %Moreover, the set semantics of $\frac{1}{\unit}f_i(\boxm) = [0, 1]$. Recall that 
  %\[ 
  %f_i(\bx)=\begin{cases}
  %             f(\bx) - i \unit, & i \unit < f(\bx) \leq (i + 1)\unit \\
  %             0, & f(\bx) \leq i\unit \\
  %             \unit, &(i+1) \unit < f(\bx)
 %           \end{cases}
%\]
%We have seen that $f(c) \leq (i-1)\unit < i\unit$, so  $\frac{1}{\unit}f_i(c) = 0$. Similarly, we have $f(d) \geq (i+2)\unit$, then $f(d) >(i+1)\unit $, so $\frac{1}{\unit}f_i(d) = 1$. Because $f(i)$ is continuous so 
%$[0, 1]\subseteq \frac{1}{\unit}f_i(\boxm)$. Also, by definition
%$\frac{1}{\unit}f_i\subseteq [0,1]$, then $\frac{1}{\unit}f_i(\boxm) = [0, 1]$.
 
%\aws{ $f(d) = u $ not $l$}

\input{ill_step4}


  This drives us to decompose the sum as follows:
  \begin{equation}\label{eq:sum}
        \sum_{i=0}^K \nn_i^\#(B)
                    \quad = \quad \underbrace{\sum_{i=0}^{p-2} \nn_i^\#(B)}_\text{Term 1} \absplus \underbrace{\sum_{i=p-1}^{p+1} \nn_i^\#(B)}_\text{Term 2} \absplus \underbrace{\sum_{i=p+2}^{q-2} \nn_i^\#(B)}_\text{Term 3} 
                    \absplus \underbrace{\sum_{i=q-1}^{q+1}\nn_i^\#(B)}_\text{Term 4} \absplus \underbrace{\sum_{i=q+2}^K \nn_i^\#(B)}_\text{Term 5}
        %&\subseteq& (0.5\epsilon, \infty)
  \end{equation}
We will analyze the five terms in~\cref{eq:sum} separately, and then take their sum to get the final result. For now, assume that $q\geq p+3$; 
the  $q\leq p+2$ case will follow easily.
\begin{enumerate}[label=(\roman*)]
    \item Term 1: $\forall i \leq p-2$, we have $p\unit \geq (i+2)\unit $. Because $l = \min f(\boxm)$ and $l\in [p\unit, (p+1)\unit)$, then $f(\boxm)\geq p\unit \geq (i+2)\unit$.% when $i \leq p-2$.
    
    From~\cref{thm:abs_slice},  $\exists u_i\in (1-\lprec, 1]$ such that $[u_i, u_i]\subseteq \nn_i^\#(\boxm) \subseteq (1-\lprec, 1]$. Then $\sum_{i=0}^{p-2} [u_i, u_i] \subseteq \sum_{i=0}^{p-2} \nn_i^\#(B)  \subseteq \sum_{i=0}^{p-2} (1-\lprec, 1]$.
%
    \[\sum_{i=0}^{p-2}[u_i, u_i] \quad \subseteq \quad  \sum_{i=0}^{p-2} \nna_i(B) \quad  \subseteq \quad (p-1)^\#\abstimes (1-\lprec, 1]\]

    \item Term 5:  $\forall i \geq q+2$, we have $(q+1)\unit \leq (i-1)\unit $. Because $u = \max f(\boxm)$ and $u\in [q\unit, (q+1)\unit)$, then $f(\boxm)< (q+1)\unit \leq (i-1)\unit$. % when $i \geq q$.
    %\aws{explain the $\unit$ part}
    
    From~\cref{thm:abs_slice},  $\exists l_i\in [0,\lprec)$ such that $[l_i, l_i]\subseteq \nna_i(\boxm) \subseteq [0, \lprec)$. Then $\sum_{i=q+2}^{K} [l_i, l_i] \subseteq \sum_{i=q+2}^{K} \nna_i(\boxm)  \subseteq \sum_{i=q+2}^{K} [0, \lprec)$.
%
    \[\sum_{i=q+2}^{K}[l_i, l_i] \quad \subseteq \quad \sum_{i=q+2}^{K} \nna_i(\boxm)  \
    \quad \subseteq \quad (K-q-1)^\#\abstimes [0, \lprec)\]

    \item Term 3: $\forall i \in [p+2, q-2]$, we have $(p+1)\unit\leq (i-1)\unit$ and $q\unit\geq (i+2)\unit$. 

    $f(c) = l < (p+1)\unit \leq (i-1)\unit$, and $f(d) = u \geq q\unit \geq (i+2)\unit$. 
    
    From~\cref{thm:abs_slice}, $\nna_i(\alpha(\{c\})) \subseteq [0, \lprec)$ and  $\nna_i(\alpha(\{d\})) \subseteq (1 - \lprec, 1]$. 
    Because $c, d\in \boxm$, $[\lprec, 1- \lprec] \subseteq \nna_i(\boxm)$.
    
    Also by~\cref{thm:abs_slice}, $\nna_i(\boxm)\subseteq [0, 1]$. Hence, $\sum_{i = p+2}^{q-2}[\lprec, 1-\lprec]\subseteq \sum_{i = p+2}^{q-2} \nna_i(\boxm) \subseteq \sum_{i = p+2}^{q-2}[0, 1]$.
    %
    \[\sum_{i = p+2}^{q-2}[\lprec, 1-\lprec] \quad \subseteq \quad \sum_{i=p+2}^{q-2} \nna_i(\boxm) \quad \subseteq \quad (q-p-3)^\#\abstimes[0, 1]\]
    
    \item Term 2: $\forall i\in [p-1, p+1]$, since we have assumed that $q\geq p+3$, 
    then $q\geq p+3\geq i+2$.
    
    Because $f(d) \geq q\unit \geq (i+2)\unit$, from~\cref{thm:abs_slice}, $\exists u_i\in (1-\lprec, 1]$ such that 
    $[u_i, u_i]\subseteq \nn_i^\#(\alpha(\{d\}))\subseteq (1-\lprec, 1]$. 
    % \aws{the previous statement does not seem to follow from theorem.
    % how come $u_i$ is precisely $\nna_i(\alpha(\{d\}))$, which can be a singleton box}
    
    Because $d\in \boxm$,  $[u_i, u_i]\subseteq \nna_i(\boxm)$.
    Hence, $[u_i, u_i]\subseteq \nna_i(B) \subseteq [0, 1]$ and $\sum_{i = p-1}^{p+1} [u_i, u_i]\subseteq \sum_{i = p-1}^{p+1}\nna_i(\boxm) \subseteq \sum_{i = p-1}^{p+1}[0, 1]$.
%
    \[\sum_{i = p-1}^{p+1}[u_i, u_i] \quad \subseteq \quad \sum_{i = p-1}^{p+1}\nna_i(\boxm) \quad \subseteq \quad 3^\#\abstimes[0, 1]\]
    
    \item Term 4: For $\forall q-1\leq i\leq q+1$, because $q\geq p+3$, we have $p+1 \leq q-2 \leq i-1$. Then $f(c) = l<(p+1)\unit\leq (i-1)\unit$. From~\cref{thm:abs_slice}, 
    $\exists l_i\in [0,\lprec)$ such that $[l_i, l_i]\subseteq \nn_i^\#(\alpha(\{c\}))\subseteq [0, \lprec)$. 
    
    Because $c\in \boxm$, $[l_i, l_i]\subseteq \nna_i(\boxm)$. Thus, 
    $[l_i, l_i]\subseteq \nna_i(\boxm)\subseteq [0, 1]$.
    
    \[\sum_{i=q-1}^{q+1}[l_{i}, l_{i}]\subseteq \sum_{i=q-1}^{q+1}\nna_{i}(\boxm) \subseteq  3^\#\abstimes[0, 1]\]
\end{enumerate}

%\aws{i like this, but maybe say what you mean by exact.}
%\paragraph{Imprecise Terms} \zw{Rewrite the whole paragraph} 

\paragraph{Step B: Sum all five cases}
% \begin{multline}
% \sum_{i=0}^{p-2}[u_i, u_i]\absplus \sum_{i=q+2}^{K}[l_i, l_i]\absplus\sum_{i = p+2}^{q-2}[\lprec, 1-\lprec]\absplus\sum_{i = p-1}^{p+1}[u_i, u_i]\absplus \sum_{i=q-1}^{q+1}[l_{i}, l_{i}] \\ 
% \subseteq \sum_{i=0}^{K} \nn_{i}^\#(\boxm)\subseteq \\ 
% (p-1)^\#\abstimes (1-\lprec, 1]\absplus(K-q-1)^\#\abstimes [0, \lprec)\absplus(q-p-3)^\#\abstimes[0, 1]\absplus 3^\#\abstimes[0, 1]\absplus 3^\#\abstimes[0,1]
% \end{multline}
%
%Notice that there is a factor $\unit$ in~\cref{eq:sum} we have not considered yet. 
We now sum up all five inequalities we derived above
to  derive an overall bound of the sum in the form 
$[L'_1, U'_1]\subseteq \sum_{i=0}^{K} \nn_{i}^\#(\boxm) \subseteq [L'_2, U'_2]$.
For example, 
\[L'_1 = \sum_{i=0}^{p-2} u_i + \sum_{i=q+2}^{K} l_i + \sum_{i = p+2}^{q-2}\lprec + \sum_{i = p-1}^{p+1}u_i + \sum_{i=q-1}^{q+1} l_i\]

%Then $L_1 = \unit L'_1$, $L_2 = \unit L'_2$, $U_1 = \unit U'_1$, $U_2 = \unit U'_2$.


Recall that, by \cref{thm:abs_slice}, $\forall i\in\{0, \ldots, K\}$, $u_i\in(1-\lprec, 1]$ and $l_i\in[0,\lprec)$. Let $\tilde{l}_i = 1-u_i$, so $\tilde{l}_i\in[0, \lprec)$.


We simplify $L_1'$, $L_2'$, $U_1'$ and $U_2'$ as follows; we list intermediate steps in supplementary materials:

\begin{itemize}
\item
     $   L'_1 = %\sum_{i=0}^{p-2}u_i + \sum_{i=q+2}^K l_i + \sum_{i = p+2}^{q-2}\lprec+\sum_{i=p-1}^{p+1}u_i+\sum_{i=q-1}^{q+1}l_{i}\\
        (p+2) + \sum_{i=0}^{p+1}(-\tilde{l}_i)+\sum_{i=q-1}^K l_i+\sum_{i = p+2}^{q-2}\lprec$

From~\cref{lem:ineq}, $\sum_{i=0}^{p+1}(-\tilde{l}_i)+\sum_{i=p+2}^{q-2}\lprec+\sum_{i=q-1}^K l_i\in [1, 1]$ 
by plugging in $-\tilde{l}_i, l_i, \lprec$ to $\eta_i$. So,
\[L'_1\in [p+1, \ p+3]\]

\item
$
        U'_1 = %\sum_{i=0}^{p-2}u_i + \sum_{i=q+2}^K l_i + \sum_{i=p+2}^{q-2}(1-\lprec)+\sum_{i=p-1}^{p+1}u_i+\sum_{i=q-1}^{q+1}l_{i}\\
        (q-1) + \sum_{i=0}^{p+1}(-\tilde{l}_i)+\sum_{i=q-1}^K l_i+\sum_{i=p+2}^{q-2}(-\lprec)
$

From~\cref{lem:ineq}, $\sum_{i=0}^{p+2}(-\tilde{l}_i)+\sum_{i=p+2}^{q-2}(-\lprec)+\sum_{i=q-1}^K l_i\in [-1, 1]$. Thus, 
%
\[U'_1\in [q-2, \ q]\]

\item
$
    L'_2 = %(p-1)(1-\lprec) = 
    (p-1)+(p-1)(-\lprec)
$

Because $\lprec \leq \frac{1}{K+1}$, and $-K\leq p-1\leq K$,
we have $(p-1)(-\lprec)\in [-1, 1]$. Hence, 
\[L'_2\in [p-2, \ p]\]

\item
$
        U'_2 = %(p-1)+(K-q-1)\lprec+(q-p-3) +3 + 3 = 
        q+2+(K-q-1)(\lprec)
$

%
Because $\lprec \leq \frac{1}{K+1}$, and $-K\leq (K-q-1)\leq K$, we have $(K-q+1)(-\lprec)\in [-1, 1]$. Then,
\[U'_2\in [q+1, \ q+3]\]

\end{itemize}

\paragraph{Step C: Analyze the bound}
%
It remains to show that $l-\delta \leq L_2\leq L_1 \leq l+\delta$ and $u-\delta \leq U_1 \leq U_2 \leq u+\delta$. 

Recall that we have set that $\delta = 3\unit$ in~\cref{sec:step1}. Also $l\in[p\unit, (p+1)\unit)$, then 
\[l-\delta < (p-2)\unit \quad\quad \text{ and } \quad\quad l+\delta\geq (p+3)\unit\] 
%
Since
$u\in[q\unit, (q+1)\unit)$, then 
\[u-\delta < (q-2)\unit \quad\quad\text{ and }\quad\quad u+\delta\geq (q+3)\unit\]


We have just analyzed $L_1'$, $L_2'$, $U_1'$ and $U_2'$ above. Now we have:
\[
    L_1 = \unit L'_1 \leq (p+3)\unit 
    \quad\quad\quad\quad 
L_2 = \unit L'_2\geq (p-2)\unit
 \]
\[U_1=\unit U'_1\geq(q-2)\unit
\quad\quad\quad\quad U_2 = \unit U'_2 \leq (q+3)\unit\]

It follows from the above inequalities that
\[
\mathhl{l-\delta} \ < \ (p-2)\unit \ \leq \  \mathhl{L_2} \leq \mathhl{L_1} \ \leq  \   (p+3)\unit \ \leq \  \mathhl{l+\delta}
\]
and 
\[\mathhl{u-\delta} \ < \ (q-2)\unit \ \leq \ \mathhl{U_1}  \leq   \mathhl{U_2} \ \leq  \ (q+3)\unit \ \leq \ \mathhl{u+\delta}
\]
This concludes the proof for the case where $q \geq p+3$.


\paragraph{Excluded case}
Previously, we have shown that Terms 1, 3, and 5 are almost precise. 
The imprecise terms can only come from Terms 2 and 4. 
If $q\leq p+2$, the only analyses that will be affected are
those of Terms 2 and 4.
Since $q\leq p+2$, we have $p+1\geq q-1$,
which means Terms 2 and 4 have potentially less sub-terms
in this case. 
Thus imprecise terms are less than the $q\geq p+3$ case and we can apply the same analysis as above and derive the same bound.

We have thus shown that the neural network $\nn$ that we construct $\delta$-abstractly approximates $f$, and therefore the AUA theorem is 
true.

\hfill\qed

%Specifically,
%when $i\in \{p-1, p+1, q-1, q+1\}$, $\nna_i(\boxm)$ are imprecise. That is, the abstract semantics of $\nna_i(\boxm)$ 
%and the collecting semantics of $f_i(\boxm)$ are obviously different. In fact, we can find exactly what 
%$f_i(\boxm)$ is for $i\in \{p-1, p+1, q-1, q+1\}$, but we only have a rough upper and lower bounds for $\nna_i(\boxm)$.

%Recall that
%\[ 
%  f_i(\bx)=\begin{cases}
%               f(\bx) - i \unit, & i \unit < f(\bx) \leq (i + 1)\unit \\
%               0, & f(\bx) \leq i\unit \\
%               \unit, &(i+1) \unit < f(\bx)
%            \end{cases}
%\]

%\begin{itemize}
%    \item \emph{Case $i = p-1$}: For $\bx\in \boxm$, $f(\bx)\geq \min f(B) = l\geq p\unit \geq ((p-1)+1)\unit$. By the definition of $f_{p-1}(\bx)$,
%    $\forall\bx\in \boxm$, we have $f_{p-1}(\bx) = \unit$. Therefore, $f_{p-1}(\boxm) = [\unit,\unit]$.
%    \item \emph{Case $i = q+1$}: 
%    For $\bx\in \boxm$, $f(\bx)\leq \max f(B) = u < (q+1)\unit$. From the definition of $f_{q+1}(\bx)$,
%    $\forall\bx\in \boxm$, we have $f_{q+1}(\bx) = 0$. Therefore, $f_{q+1}(\boxm) = [0,0]$.
%    \item \emph{Cases  $i = p+1$ or $i = q-1$}: Because $f(c) = l <(p+1)\unit\leq i\unit$, then $f_i(c) = 0$.
%    Similarly, $f(d)=u\geq q\unit\geq (i+1)\unit$, so $f_i(d) = \unit$. By the continuity and definition of $f_i(\bx)$,
%    we can conclude that $f_{i}(\boxm) = [0,\unit]$.
%\end{itemize}

% If the corresponding $\nna_i(\boxm)$ are precise, then we should have got 
% $[\approx 1,\approx 1]\subseteq \nna_{p-1}(\boxm)\subseteq[\approx 1, \approx 1]$,
% $[\approx 0, \approx 1]\subseteq \nna_{p+1}(\boxm)\subseteq[\approx 0, \approx 1]$, 
% $[\approx 0, \approx 1]\subseteq \nna_{q-1}(\boxm)\subseteq[\approx 0, \approx 1]$,
% and $[\approx 0, \approx 0]\subseteq \nna_{q+1}(\boxm)\subseteq[\approx 0, \approx 0]$.

%but $\nna_i(\boxm)$ are different from the corresponding 
%set semantics for $i\in \{p-1, p+1, q-1, q+1\}$.



%For example, if $q = p+j$ for $j\in\{0, 1, 2\}$, then 
%\[
%    \sum_{i=0}^K \nn_i^\#(B) = \sum_{i=0}^{p-2} \nn_i^\#(B) \absplus \sum_{i=p-1}^{p+j-2} \nn_i^\#(B) \absplus \nn_{p+1}^\#(B) \absplus \sum_{i=q+2-j}^{q+1}\nn_i^\#(B) \absplus \sum_{i=q+2}^K \nn_i^\#(B) 
%\] 
%The analysis for all terms except for $\nn_{p+1}^\#(B)$ is the same. In the above analysis, only cases 4 and 5 rely on the assumption $p+3 \leq q$. Now if we have $q = p+2$:
%\aws{it's confusing: what are we analyzing the example case $q=p+2$ or the general case $q\leq p+2$?
%Just show the general case.}
%\begin{enumerate}
%    \item If $i = p-1$ or $i = p$, $q= p+2\geq i+2$, then $f(d) \geq q\unit \geq (i+2)\unit$, as in the original case. Hence the analysis is the same.
%    \item If $i = q$ or $i = q+1$, $p+1 = q-1 \leq i-1$, then $f(c) = l<(p+1)\unit\leq (i-1)\unit$, as in the original case. Hence the analysis is the same.
%\end{enumerate}

%The only remaining imprecise term is $\nn_{p+1}^\#(B)$, and we only have $[a, a]\subseteq \nn_{p+1}^\#(B)\subseteq [0, 1]$ where $a\in [0, 1]$. However, because terms in case 4 and 5 are less, for example, in case 4, 
%if $q\geq p+3$, there are 3 terms, but now we only have 2 terms, we already have a tighter bound. Then $\forall a\in [0,1]$, if we apply the same analysis as above, we can get the same bound.
%\aws{this paragraph doesn't make sense.}




==> squashable.tex <==
\section{Squashable and Step Functions}\label{sec:squashable}
In this section, we will show some constructions using squashable and step functions. This is the key idea of the whole paper, and essential for proving the IUA and the hardness of range approximation theorem. We believe that these constructions are important in understanding the computational and formal properties of neural networks in the future.

\input{ill_step2_bump}

\paragraph{Step Function}
A step function is
\[ \step(x) = \left\{ \begin{array}{ll}
    1, & \mbox{$x > 0$}\\
    0, & \mbox{$x \leq 0$}\end{array} \right.\]

One can view the step function as the indication of whether $x$ is a positive number. The step function can be used to build indicator functions, which is a fundamental tool in mathematical analysis. For example, the standard way of defining integration with respect to the probability measure is using the summation of indicator functions~\citep{probability}. Also, neural networks with step functions as the activation function can encode boolean formula.

\paragraph{Squashable Function}
Squashable functions do not have a concrete formula, as it is a very expressive class of functions. All we know is that it is monotonic and has both left and right limits (see~\cref{def:activation}). Proving the properties of neural network with squashable functions might appear a challenging task.

However, the key observation is that if we dilate $\act$ properly, i.e., multiply the input with a large number $\dilate$ to get $\act(\dilate x)$, we will obtain an approximation of the step function.
See~\cref{fig:step_fn,fig:dilated_sigmoid} on how one can use the sigmoid function to approximate the step function.

\paragraph{Indicator Function}
An indicator function associated with a set $S\subset \R^m$ is defined as
\[\bump_S = \left\{ \begin{array}{ll}
    1, & \mbox{$\bx \in S$}\\
    0, & \mbox{$\bx \not\in S$} \end{array} \right.\]
Note how the value is $1$ if $\bx$ is in the set $S$,
and $0$ otherwise.

The framework developed by~\citet{univ_cert} to show that neural networks with $\relu$ activations is interval universal approximator can be viewed as a summation of indicator functions. The underlying sets are boxes in $\R^m$. The indicator construction in~\citep{univ_cert} uses the $\min$ function construction from~\citep{arora2018understanding}, which was to show that $\relu$ network can construct any piecewise linear function. 

We adapt the framework, and use a different construction to build the indicator function from step functions. For example,
\[\step(x) - \step(x-1)\]
returns 1 for $x \in (0,1]$, and 0 otherwise. See~\cref{fig:bump,fig:dilated_sigmoid_bump} for illustrations of the (approximating) indicator function on $(0,1]$.

\paragraph{Encoding Boolean Formula}
A boolean formula is a composition of operators $\lnot$, $\land$ and $\lor$ and variables that take values $\{0,1\}$. To simulate a boolean formula, for each variable, we can build a input node corresponding to the variable. We only need to encode the logical operators. 
\begin{enumerate}
    \item For $\lnot \phi_x$, we only need to use $1- X$, where $X$ is the neural network node corresponds to the expression $\phi_x$.
    \item For $\phi_x\land \phi_y$, we can use $\step(X+Y-1.5)$. For $X$ and $Y$ that takes values in $\{0,1\}$, $\step(X+Y-1.5)$ evaluates to $1$ only when both $X$ and $Y$ are $1$.
    \item For $\phi_x\lor \phi_y$, we can use $\step(X+Y-0.5)$. For $X$ and $Y$ that takes values in $\{0,1\}$, $\step(X+Y-0.5)$ evaluates to $0$ only when both $X$ and $Y$ are $0$.
\end{enumerate}

One can then build a neural network that encodes a boolean formula recursively according to the syntactical composition of the formula. In~\cref{sec:hardness}, we will consider boolean formulas of special forms, i.e., $3\CNF$ (conjunction normal form) and $3\DNF$ (disjunction normal form). We will present encodings of the $3\CNF$ and $3\DNF$ formulas using neural networks with squashable functions, and the construction essentially captures the computation of corresponding logical operators.


\paragraph{Remark} As we shall see later, the step function formulation serves as the intuition for understanding the neural network with squashable activations. However, because we do not have the perfect step function as the activation, and the values are continuous rather than $\{0,1\}$, to rigorously prove the results, we need to carefully control the imprecision introduced by the approximation of squashable functions, and the construction that works for discrete values might not work for continuous values directly. Nevertheless, one can expect the formal property of neural networks with squashable activations will not be fundamentally different from its boolean formula or step-function neural network counterparts. Moreover, the step function gadget can still guide the design for the network with squashable functions. In fact, we will show that the complexity result in~\citep{katz2017reluplex} that it is $\NP$-hard to verify \footnote{We follow the definition of verifying properties of neural networks in~\citep{katz2017reluplex}, as deciding whether the conjunction of linear constraints on the input and output of the network is satisfiable.} a neural network can be easily proved using the squashable function idea, and as a corollary of the result we will present.
